An Adaptive Empirical Bayesian Method for Sparse Deep Learning

We propose a novel adaptive empirical Bayesian method for sparse deep learning, where the sparsity is ensured via a class of self-adaptive spike-and-slab priors. The proposed method works by alternatively sampling from an adaptive hierarchical posterior distribution using stochastic gradient Markov Chain Monte Carlo (MCMC) and smoothly optimizing the hyperparameters using stochastic approximation (SA). We further prove the convergence of the proposed method to the asymptotically correct distribution under mild conditions. Empirical applications of the proposed method lead to the state-of-the-art performance on MNIST and Fashion MNIST with shallow convolutional neural networks and the state-of-the-art compression performance on CIFAR10 with Residual Networks. The proposed method also improves resistance to adversarial attacks.

==> NIPS 2019 An Adaptive Empirical Bayesian Method for Sparse Deep Learning -arXiv/acknow.tex <==

$\newline$
\textbf{Acknowledgments}

We would like to thank Prof. Vinayak Rao, Dr. Yunfan Li and the reviewers for their insightful comments. We acknowledge the support from the National Science Foundation (DMS-1555072, DMS-1736364, DMS-1821233 and DMS-1818674) and the GPU grant program from NVIDIA.

==> NIPS 2019 An Adaptive Empirical Bayesian Method for Sparse Deep Learning -arXiv/concl.tex <==
% about running time, from Chen 2014, when n is large, restrict all the matrices to be diagonal, resulting in the same time complexity with SGLD
We propose a novel AEB method to adaptively sample from hierarchical Bayesian DNNs and optimize the spike-and-slab priors, which yields a class of scalable adaptive sampling algorithms in DNNs. We prove the convergence of this approach to the asymptotically correct distribution. By adaptively searching and penalizing the over-fitted parameters, the proposed method achieves higher prediction accuracy over the traditional SG-MCMC methods in both simulated examples and real applications and shows more robustness towards adversarial attacks. Together with the magnitude-based weight pruning strategy and simulated annealing, the AEB-based method,  A-SGHMC-SA, obtains the state-of-the-art performance in model compression. %For larger networks, longer training time might be needed. Existing techniques, such as gradient noise control and temperature tuning, for accelerating SG-MCMC simulations should also be helpful to this proposed method.

%\footnote{Code will be available upon request.} %Simulated examples and real applications show the robustness of our proposed method over the traditional SG-MCMC methods and the resistance to over-fitting.

% Interesting future directions include applying SG-MCMC-SA to active learning to learn from datasets of smaller size and proving posterior consistency and the consistency of variable selection under various shrinkage priors concretely.

==> NIPS 2019 An Adaptive Empirical Bayesian Method for Sparse Deep Learning -arXiv/convergence.tex <==


% % Uncertainty quantification of large systems is extremely time-consuming. In the framework of deep neural networks, it is necessary to propose an efficient sampling method for Bayesian deep learning models with latent variables. It is natural to use a Gibbs sampler in SGLD to sample latent variables $\bm{H}$ in sequence (\ref{eq:17}) and obtain an "auxiliary" ergodic Markov Chain \citep{George93}: 
% % \begin{equation}
% % \label{eq:17}
% % \bm{\beta}^{(1)}, \bm{H}^{(1)}; \bm{\beta}^{(2)}, \bm{H}^{(2)}; \bm{\beta}^{(3)}, \bm{H}^{(3)}; \ldots
% % \end{equation}
% % However, this strategy has been criticized \citep{Rockova14} due to its lack of efficiency in sampling and practicality in large-scale problems. 

% In this section, we study the convergence of the algorithm when the network is not pruned, we view $(\bm{\rho}, \sigma, \bm{\tau}, \delta)$ as a vector $\bm{\theta}$ and formulate our algorithm as follows: % Liang's version
% % Extension of EMVS to DNN is nontrivial since we cannot get the closed form solution of $\bm{\beta}$ as in EMVS. In addition, the improper initialization of hyperparameters and the noise from stochastic optimization error strongly bias the updates of latent variables, which either causes them to rapidly converge to arbitrarily poor local optima or makes the whole algorithm diverge. To tackle this issue, we replace the M-step by SG-MCMC with the prior hyperparameters tuned via stochastic approximation \citep{Albert90} (Appendix A.2): % Liang's version % Liang, Deng's combination
% % Extension of EMVS to DNN is nontrivial since we cannot get the closed form solution of $\bm{\beta}$ as in EMVS. In addition, the improper initialization of hyperparameters and the noise from stochastic optimization error strongly bias the updates of latent variables, which either causes them to rapidly converge to arbitrarily poor local optima or makes the whole algorithm diverge. To make sure the convergence of SG-MCMC in models with latent variables, we propose to use the idea of stochastic approximation \citep{Albert90} (see details in Appendix A.2) to control the growth of approximation error by iteratively updating the latent variables: % Deng's version
% \begin{equation}
% \begin{split}
% \label{eq:0000}
% \bm{\beta}^{(k+1)}&=\bm{\beta}^{(k)} + \epsilon^{(k)} \nabla_{\bm{\beta}} \tilde{L}(\bm{\beta}^{(k)}, \bm{\theta}^{(k)})+\tilde{\bm{\eta}}^{(k)}, \\
% \bm{\theta}^{(k+1)}&=\bm{\theta}^{(k)}+\omega^{(k+1)}\left( g_{\bm{\theta}^{(k)}}(\bm{\beta}^{(k+1)})-\bm{\theta}^{(k)}\right), \\
% \end{split}
% \end{equation}
% where $\tilde{\bm{\eta}}^{(k)}\sim\mathcal{N}(0, 2\epsilon^{(k)}/\tau\bm{I})$,  $g_{\bm{\theta}}(\cdot)$ is the mapping detailed in Eq.(\ref{eq:10}), Eq.(\ref{eq:11}), Eq.(\ref{eq:13}) and Eq.(\ref{eq:14}) to derive $\bm{\theta}$ based on the current $\bm{\beta}$, the step size $\omega^{(k)}$ can be set as $A(k+Z)^{-\alpha}$ with $\alpha\in (0.5, 1]$. The interpretation of this algorithm is that we sample $\bm{\beta}^{(k+1)}$ from $\tilde{L}(\bm{\beta}^{(k)}, \bm{\theta}^{(k)})$ and adaptively optimize the expectation of $\bm{\theta}^{(k+1)}$. 
% % We expect to obtain an augmented sequence as follows: 
% % \begin{equation}
% % \label{eq:17}
% % \bm{\beta}^{(1)}, \bm{\theta}^{(1)}; \bm{\beta}^{(2)}, \bm{\theta}^{(2)}; \bm{\beta}^{(3)}, \bm{\theta}^{(3)}; \ldots
% % \end{equation}

% To provide the $L^2$ upper bound for SGLD-SA, we first lay out the following assumptions:
% \begin{assumption}[Step size]
% \label{ass1}
% $\{\omega^{(k)}\}_{k\in \mathrm{N}}$ is a positive decreasing sequence of real numbers such that
% \begin{equation}
% \begin{split}
% \label{a1}
% &\omega^{(k)}\rightarrow 0, \ \ \sum_{k=1}^{\infty} \omega^{(k)}=+\infty.
% \end{split}
% \end{equation}
% \end{assumption}

% \begin{assumption}[Smoothness]
% \label{ass_2_1}
% $L(\bm{\beta}, \bm{\theta})$ is $G$-smooth with $G>0$, i.e. for any $\bm{\beta}, \bm{\iota}\in \bm{B}$, $\bm{\theta}, \bm{\upsilon}\in\bm{\Theta}$.
% \begin{equation}
% \begin{split}
% \label{ass_2_1_eq}
% \|\nabla_{\bm{\beta}} L(\bm{\beta}, \bm{\theta})-\nabla_{\bm{\beta}} L(\bm{\iota}, \bm{\upsilon})\|\leq G\|\bm{\beta}-\bm{\iota}\|+G\|\bm{\theta}-\bm{\upsilon}\|. 
% \end{split}
% \end{equation}
% \end{assumption}

% \begin{assumption}[Dissipative] There exist constants $m>0, b\geq 0$, s.t. for all $\bm{\beta} \in \bm{\beta}$ and $\bm{\theta} \in \bm{\Theta}$, we have 
% \label{ass_dissipative}
% \begin{equation}
% \label{eq:01}
% \langle \nabla_{\bm{\beta}} L(\bm{\beta}, \bm{\theta}), \bm{\beta}\rangle\leq b-m\|\bm{\beta}\|^2.
% \end{equation}
% \label{as:2_2}
% This condition is essential to induce ergodicity.  \citep{mattingly02, Xu18}, which means that a Markov process is able to move inwards on average.
% \end{assumption}

% \begin{assumption}[Gradient condition] The stochastic noise $\bm{\chi}^{(k)}$, which equals $\nabla_{\bm{\beta}}\tilde L(\bm{\beta}^{(k)}, \bm{\theta}^{(k)})-\nabla_{\bm{\beta}} L(\bm{\beta}^{(k)}, \bm{\theta}^{(k)})$, is a white noise and is independent with each other.
% \begin{equation}
% \begin{split}
% \label{eq:19}
% \E[\bm{\chi}^{(k)}|\mathcal{\bm{F}}^{(k)}]&=0.\\
% \end{split}
% \end{equation}
% For constants $M, B>0$, the noise scale is bounded by
% \begin{equation}
% \begin{split}
% \label{eq:19_11}
% \E\|\bm{\chi}\|^2 \leq M\E\|\bm{\beta}\|^2+M\E\|\bm{\theta}\|^2+B.\\
% \end{split}
% \end{equation}
% \label{as:1}
% \vspace{-2em}
% \end{assumption}
% We then show that both $\bm{\beta}$ and $\bm{\theta}$ are bounded in $L^2$ and present the details in Appendix B.1. 
% \begin{lemma}[Uniform $L^2$ bound]
% \label{lemma:1}
% For all $\ 0<\epsilon<\operatorname{Re}(\tfrac{m-\sqrt{m^2-2M(M+1)}}{2M(M+1)})$, there exist $G, \overline{G}>0$ such that
% $\sup \E\|\bm{\beta}_k\|^2 \leq G$ and $\sup \E\|\bm{\theta}_k\|^2 \leq \overline{G}$, where $G=\|\bm{\beta}_0\|^2 + \tfrac{1}{m}(b+B(M+1)+\tau d)$ and $\overline{G}=MG+B$.\footnote{Here we assume $\bm{\beta}\in \mathbb{R}^d$}
% \end{lemma}

% The uniform $L^2$ bound is crucial to show the convergence for the latent variables.

% \begin{theorem}[$L^2$ convergence rate]
% \label{th:1}
% For any $\alpha\in (0, 1]$, under assumptions in Appendix B.1, the algorithm satisfies: there exists a constant $\lambda$ such that
% \begin{equation*}
% \begin{split}
% \E\left[\|\bm{\theta}^{(k)}-\bm{\theta}^*\|^2\right]\leq \lambda\omega^{(k)},
% \end{split}
% \end{equation*}
% \end{theorem}
% where $\omega^{(k)}=A(k+Z)^{-\alpha}$ for some positive $A$ and $Z$.

% \begin{corollary}
% \label{cor:1}
% Given fixed stepsize $\epsilon$, the distribution of $\bm{\beta}^{(k)}$ converges weakly to the invariant distribution $e^{\tau L(\bm{\beta}, \bm{\theta}^*)}$ with rate $\alpha\in (0, 1]$ as $\epsilon\rightarrow 0$.
% \end{corollary}

% The key to guaranteeing the consistency of the latent variable estimators is from the theory of SA and the fact of $\sum_{i=1}^{\infty} \omega^{(i)}=\infty$. The smooth update of the latent variables makes the algorithm robust to bad hyperparameters and is more likely to avoid entrapment in poor local optima. The non-convex optimization of SG-MCMC \citep{Maxim17, Yuchen17, Xu18} with suitable temperature or cooling schedules ensures the robust optimization of the latent variables. Because SGHMC proposed by \citet{Chen14} is essentially a second-order Langevin dynamics and yields a stationary distribution given an accurate estimation of the error variance from the stochastic gradient, the convergence of SGLD-SA also applies to SGHMC-SA.


% \begin{algorithm}[tb]
%    \caption{SGLD-SA with spike and slab priors}
%    \label{alg: SGLD-EM}
% \begin{algorithmic}
%    \State{\textbf{Inputs:} $\{\epsilon^{(k)}\}_{k=1}^{\mathcal{T}}$, $\{\omega^{(k)}\}_{k=1}^{\mathcal{T}}$, $\tau$, a, b, $\nu$, $\lambda$, $v_0$, $v_1$}
%    \State{\textbf{Outputs:} $\{\bm{\beta}^{(k)}\}_{k=1}^{\mathcal{T}}$}
%    \State{\textbf{Initialize:} $\bm{\beta}^{(1)}$, $\bm{\rho}^{(1)}$, $\bm{\kappa}^{(1)}$, $\sigma^{(1)}$ and $\delta^{(1)}$ from scratch}
%    \For{$k \leftarrow 1:\mathcal{T}$}
%    \State{Sample mini-batch $\mathcal{B}^{(k)}$}
%    \State{\textbf{Sampling}}
% %    \State{$\bm{\beta}^{(k+1)}\leftarrow\bm{\beta}^{(k)} + \epsilon^{(k)} \nabla_{\bm{\beta}} {\pi}(\bm{\beta}^{(k)}, \sigma^{(k)}, \delta^{(k)}|\mathcal{B}^{(k)})+\sqrt{2\epsilon^{(k)} T^{-1}}\bm{\eta}^{(k)},\ \where\ \bm{\eta}^{(k)} \sim \mathcal{N}(\bm{0}, \bm{I})$}
%    \State{$\bm{\beta}^{(k+1)}\leftarrow\bm{\beta}^{(k)} + \epsilon^{(k)} \nabla_{\bm{\beta}}  Q(\bm{\beta}, \sigma, \delta|\bm{\beta}^{(k)}, \sigma^{(k)}, \delta^{(k)})+\mathcal{N}({0, 2\epsilon^{(k)} \tau^{-1}})$}
%    \State{\textbf{Optimization}}
%    \State{Compute $\bm{\rho}^{(k+1)}$ in Eq.(\ref{eq:10}), perform SA: $\bm{\rho}^{(k+1)}\leftarrow (1-\omega^{(k+1)}) \bm{\rho}^{(k)}+\omega^{(k+1)} \bm{\rho}^{(k+1)}$}
%    \State{Compute $\bm{\kappa}^{(k+1)}$ in Eq.(\ref{eq:11}), perform SA: $\bm{\kappa}^{(k+1)}\leftarrow (1-\omega^{(k+1)}) \bm{\kappa}^{(k)}+\omega^{(k+1)} \bm{\kappa}^{(k+1)}$}
%    \State{Compute $\sigma^{(k+1)}$ in Eq.(\ref{eq:13}), perform SA: $\sigma^{(k+1)}\leftarrow(1-\omega^{(k+1)}) \sigma^{(k)}+\omega^{(k+1)} \sigma^{(k+1)}$}
%    \State{Compute $\delta^{(k+1)}$ in Eq.(\ref{eq:14}), perform SA: $\delta^{(k+1)}\leftarrow(1-\omega^{(k+1)}) \delta^{(k)}+\omega^{(k+1)} \delta^{(k+1)}$}
%    \EndFor
% \end{algorithmic}
% \end{algorithm}


==> NIPS 2019 An Adaptive Empirical Bayesian Method for Sparse Deep Learning -arXiv/exps.tex <==
\subsection{Simulation of Large-p-Small-n Regression}
We conduct the linear regression experiments with a dataset containing $n=100$ observations and $p=1000$ predictors. $\mathcal{N}_p(0, \bm{\Sigma})$ is chosen to simulate the predictor values $\bm{X}$  (training set) where $\bm{\Sigma}=(\Sigma)_{i,j=1}^p$ with $\Sigma_{i,j}=0.6^{|i-j|}$. Response values $\bm{y}$ are generated from $\bm{X}\bm{\beta}+\bm{\eta}$, where $\bm{\beta}=(\beta_1,\beta_2,\beta_3,0,0,...,0)'$ and $\bm{\eta}\sim \mathcal{N}_n(\bm{0}, 3 \bm{I}_n)$. We assume $\beta_1\sim \mathcal{N}(3, \sigma_c^2)$, $\beta_2\sim \mathcal{N}(2, \sigma_c^2)$, $\beta_3\sim \mathcal{N}(1, \sigma_c^2)$,  $\sigma_c=0.2$. We introduce some hyperparameters, but most of them are uninformative. We fix $\tau=1, \lambda=1, \nu=1, v_1=10, \delta=0.5, b=p$ and set $a=1$.  The learning rate follows $\epsilon^{(k)}= 0.001\times k^{-\frac{1}{3}}$, and the step size is given by $\omega^{(k)}=10\times (k+1000)^{-0.7}$.  We vary $v_0$ and $\sigma$ to show the robustness of SGLD-SA to different initializations. In addition, to show the superiority of the adaptive update, we compare SGLD-SA with the intuitive implementation of the EMVS to SGLD and refer to this algorithm as SGLD-EM, which is equivalent to setting $\omega^{(k)}:=1$ in SGLD-SA. To obtain the stochastic gradient, we randomly select 50 observations and calculate the numerical gradient. SGLD is sampled from the same hierarchical model without updating the latent variables.

%Sensitivity analysis shows that three hyperparameters are important: $v_0$, $a$ and $\sigma$, which are used to identify and regularize the over-fitted space. 

We simulate $500,000$ samples from the posterior distribution, and also simulate a test set with 50 observations to evaluate the prediction.  As shown in Fig.\ref{fig:lr} (d), all three algorithms are fitted very well in the training set, however, SGLD fails completely in the test set (Fig.\ref{fig:lr} (e)), {indicating the over-fitting problem of SGLD without proper regularization when the latent variables are not updated}. Fig.\ref{fig:lr} (f) shows that although SGLD-EM successfully identifies the right variables, the estimations are lower biased. The reason is that SGLD-EM fails to regulate the right variables with $L_2$ penalty, and $L_1$ leads to a greater amount of shrinkage for $\bm{\beta}_1$, $\bm{\beta}_2$ and $\bm{\beta}_3$ (Fig. \ref{fig:lr} (a-c)), {implying the importance of the adaptive update via SA in the stochastic optimization of the latent variables}. In addition, from Fig.~\ref{fig:lr}(a), Fig. \ref{fig:lr}(b) and Fig.\ref{fig:lr}(c), we see that SGLD-SA is the only algorithm among the three that quantifies the uncertainties of $\beta_1$, $\beta_2$ and $\beta_3$ and always gives the best prediction as shown in Table.\ref{Linear_regression_UQ_test}. We notice that {SGLD-SA is fairly robust to various hyperparameters}.

For the simulation of SGLD-SA in logistic regression and the evaluation of SGLD-SA on UCI datasets, we leave the results in Appendix C and D.

\begin{table*}[t]  % Linear regression with UQ pars
\caption{Predictive errors in linear regression based on a test set considering different $v_0$ and $\sigma$}
\label{Linear_regression_UQ_test}
\begin{center}
\begin{small}
% \scriptsize
\begin{sc}
\begin{tabular}{lccccr}
\toprule
MAE / MSE & $v_0$=$0.01,\sigma$=2 & $v_0$=$0.1, \sigma$=2 & $v_0$=$0.01,\sigma$=1 &  $v_0$=$0.1, \sigma$=1 &\\
\midrule %% testing
SGLD-SA     & \textbf{1.89} / \textbf{5.56}  & \textbf{1.72} / \textbf{5.64}  & \textbf{1.48} / \textbf{3.51} & \textbf{1.54} / $\ $\textbf{4.42} &\\
SGLD-EM        & 3.49 / 19.31  & 2.23 / 8.22 & 2.23 / 19.28 & 2.07 / $\ $6.94 &\\
SGLD        & 15.85 / 416.39 & 15.85 / 416.39 & 11.86 / 229.38 & 7.72 / 88.90 &\\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vspace{-1em}
\end{table*}



\begin{figure*}[!ht]
  \centering
  \subfigure[Posterior estimation of $\beta_{1}$.]{\includegraphics[scale=0.25]{figures/reg_a.pdf}}\label{fig: 2a}
  \subfigure[Posterior estimation of $\beta_{2}$.]{\includegraphics[scale=0.25]{figures/reg_b.pdf}}\label{fig: 2b}
  \subfigure[Posterior estimation of $\beta_{3}$.]{\includegraphics[scale=0.25]{figures/reg_c.pdf}}\label{fig: 2c}
  \subfigure[Training performance.]{\includegraphics[scale=0.25]{figures/reg_d.pdf}}\label{fig: 2d}
  \subfigure[Testing performance.]{\includegraphics[scale=0.25]{figures/reg_e.pdf}}\label{fig: 2e}
  \subfigure[Posterior mean vs truth.]{\includegraphics[scale=0.25]{figures/reg_f.pdf}}\label{fig: 2f}
  \caption{Linear regression simulation when $v_0=0.1$ and $\sigma=1$.}
  \label{fig:lr}
  \vspace{-1em}
\end{figure*}


% Furthermore, as a byproduct of uncertainty test in Section 4.3, we also applied our framework to classify cats and dogs from Kaggle in Section 4.1. The first 20000 images of dog and cat images are used for training, the following 4000 for testing and the rest are used in Section 4.3. \textcolor{red}{OJO}The second DNN we used is the first mentioned CNN architecture in Keras Blog. We didn't tune our hyperparameters and just applied the same settings as in our first DNN. We also explored the possibility of adapting our framework to the pretrained VGG16 \citep{Simonyan16} network and do fine-tuning as suggested, a good performance can be achieved after 100 epochs to give accuracy $\sim$97\% within 3 hours using GPU 1080 Ti.


\subsection{Classification with Auto-tuning Hyperparameters}
\label{sec: mnist}

% It has 2 convolutional layers with a 2 $\times$ 2 max pooling after each layer and a 2-layer fully-connected layer \citep{Jarrett09}. The filter size in the convolutional layers is 5 $\times$ 5 and the feature maps are set to be 32 and 64, respectively. The fully-connected layers (FC) have 200 hidden nodes and 10 outputs. We use the rectified linear unit (ReLU) as the activation function between layers and employ a cross-entropy loss. 

The following experiments are based on non-pruning SG-MCMC-SA, the goal is to show that auto-tuning sparse priors are useful to avoid over-fitting. The posterior average is applied to each Bayesian model. We implement all the algorithms in Pytorch \citep{paszke2017}. The first DNN is a standard 2-Conv-2-FC CNN model of 670K parameters (see details in Appendix D.1).

%: It has two convolutional layers with a 2 $\times$ 2 max pooling after each layer and two fully-connected layers. The filter size in the convolutional layers is 5 $\times$ 5 and the feature maps are set to be 32 and 64, respectively  \citep{Jarrett09}. The fully-connected layers (FC) have 200 hidden nodes and 10 outputs. We use the rectified linear unit (ReLU) as the activation function between layers and employ a cross-entropy loss. 
The first set of experiments is to compare methods on the same model without using data augmentation (DA) and batch normalization (BN) \citep{Ioffe15}. We refer to the general CNN without dropout as {Vanilla}, with 50\% dropout rate applied to the hidden units next to FC1 as {Dropout}. %(DropConnect is not tested due to its similarity to Dropout). 

Vanilla and Dropout models are trained with Adam \citep{Kingma14} and Pytorch default parameters (with learning rate 0.001). We use SGHMC as a benchmark method as it is also sampling-based and has a close relationship with the popular momentum based optimization approaches in DNNs. {SGHMC-SA} differs from {SGHMC} in that {SGHMC-SA} keeps updating SSGL priors for the first FC layer while they are fixed in {SGHMC}. We set the training batch size $n=1000$, $a,b=p$ and $\nu,\lambda=1000$. The hyperparameters for SGHMC-SA are set to $v_0=1, v_1=0.1$ and $\sigma=1$ to regularize the over-fitted space. The learning rate is set to $5\times 10^{-7}$, and the step size is $\omega^{(k)}= 1\times (k+1000)^{-\frac{3}{4}}$. We use a thinning factor 500 to avoid a cumbersome system. Fixed temperature can also be powerful in escaping ``shallow" local traps \citep{Yuchen17}, our temperatures are set to $\tau=1000$ for MNIST and $\tau=2500$ for FMNIST.

%  The total sample size $N$ in Eq.(\ref{factor}) is set to $600,000$ instead of $60,000$.\footnote{Due to the use of DA in some experiments, we unify this number as $N=600,000$} 

% The results are averaged over 5 repeated experiments for a comprehensive evaluation. 
The four CNN models are tested on MNIST and Fashion MNIST (FMNIST) \citep{Xiao17} dataset. Performance of these models is shown in Tab.\ref{tab:classi}. Compared with SGHMC, our SGHMC-SA outperforms SGHMC on both datasets. We notice the posterior averages from SGHMC-SA and SGHMC obtain much better performance than Vanilla and Dropout. {Without using either DA or BN, SGHMC-SA achieves {99.59}\% which outperforms some state-of-the-art models}, such as Maxout Network (99.55\%) \citep{Goodfellow13} and pSGLD (99.55\%) \citep{Li16} . In F-MNIST, SGHMC-SA obtains 93.01\% accuracy, outperforming all other competing models. %such as stochastic pooling (99.53\%) \citep{Zeiler13}, Maxout Network (99.55\%) \citep{Goodfellow13} and pSGLD (99.55\%) \citep{Li16} . In F-MNIST, SGHMC-SA obtains 93.01\% accuracy, outperforming all other competing models. 

To further test the performance, we apply DA %\footnote[1]{For FMNIST and CIFAR10, random erasing {\citep{Zhong17}} is also used in DA} 
and BN to the following experiments (see details in Appendix D.2) and refer to the datasets as $\text{DA-MNIST}$ and $\text{DA-FMNIST}$. All the experiments are conducted using a 2-Conv-BN-3-FC CNN of 490K parameters. %:  It has two convolutional layers with a $2\times2$ max pooling after each layer and three fully-connected layers with batch normalization applied to the first FC layer. The filter size in the convolutional layers is $4\times4$ and the feature maps are both set to 64. We use $256\times64\times10$ fully-connected layers. 
Using this model, we obtain the {state-of-the-art 99.75\%} on $\text{DA-MNIST}$ (200 epochs) and {94.38}\% on $\text{DA-FMNIST}$ (1000 epochs) as shown in Tab. \ref{tab:classi}. The results are noticeable, because posterior average is only conducted on a single shallow CNN. 
%We also conduct the experiments based on the ensemble of five networks and refer them as $\lowercase{a}\text{MNIST-5}$ and $\lowercase{a}\text{FMNIST-5}$ in Tab. \ref{tab:classi}. 
%We achieve \textbf{99.79\% on $\lowercase{a}\text{MNIST-5}$} using 5 small Bayesian neural networks each with 2 thinning samples (4 thinning samples in $\lowercase{a}\text{FMNIST-5}$), which is comparable with the \textbf{state-of-the-art performance} \citep{Liwan13}. 
% as shown in Tab.\ref{mnist-table}

% \begin{table}[t]
% \caption{Classification accuracy from a single model}
% \label{data-table}
% \begin{center}
% \begin{small}
% \begin{sc}
% \label{tab:classi}
% \begin{tabular}{lccccr}
% \toprule
% Dataset & MNIST & F-MNIST & MNIST-DA & F-MNIST-DA &  \\
% \midrule
% Vanilla    & 99.24 (99.31) & 92.53 (92.73) \\
% Dropout    & 99.33 (99.38) & 92.60 (92.81)  \\
% \midrule
% SGHMC & 99.45 (99.55) & 92.65 (92.85) \\
% SGHMC-SA    & \textbf{99.52 (99.60)} & \textbf{92.71 (93.01)} & \textbf{99.71 (99.75)} & \textbf{(94.11) 94.38} \\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \end{table}


% \begin{table}[t]
% \caption{Classification accuracy using shallow networks}
% \label{data-table}
% \begin{center}
% % \scriptsize
% \begin{sc}
% \label{tab:classi}
% \begin{tabularx}{0.7\textwidth}{lcccc}
% \toprule
% Dataset & $\text{MNIST}$ & $\text{DA-MNIST}$ &  $\text{FMNIST}$ & $\text{DA-FMNIST}$\\
% \midrule
% Vanilla     & 99.31 & 99.54  & 92.73 & 93.14  \\
% Dropout     & 99.38 & 99.56  & 92.81 & 93.35  \\
% \midrule
% SGHMC       & 99.47 & 99.63  & 92.88 & 94.29   \\
% \textbf{SGHMC-SA}    & \textbf{99.59} & \textbf{99.75} & \textbf{93.01} & \textbf{94.38}  \\
% \bottomrule
% \end{tabularx}
% \end{sc}
% \end{center}
% \vspace{-1.5em}
% \end{table}

\begin{table}[t]
\caption{Classification accuracy using shallow networks}
\label{data-table}
\begin{center}
% \scriptsize
\small
\begin{sc}
\label{tab:classi}
\begin{tabularx}{0.7\textwidth}{lcccc}
\toprule
Dataset & $\text{MNIST}$ & $\text{DA-MNIST}$ &  $\text{FMNIST}$ & $\text{DA-FMNIST}$\\
\midrule
Vanilla     & 99.31 & 99.54  & 92.73 & 93.14  \\
Dropout     & 99.38 & 99.56  & 92.81 & 93.35  \\
\midrule
SGHMC       & 99.47 & 99.63  & 92.88 & 94.29   \\
\textbf{SGHMC-SA}    & \textbf{99.59} & \textbf{99.75} & \textbf{93.01} & \textbf{94.38}  \\
\bottomrule
\end{tabularx}
\end{sc}
\end{center}
\vspace{-2em}
\end{table}

% \begin{table}[t]
% \caption{Classification accuracy on MNIST using shallow networks}
% \label{data-table}
% \begin{center}
% \begin{small}
% \begin{sc}
% \label{tab:classi}
% \begin{tabular}{lccc}
% \toprule
% Dataset & $\text{MNIST}$ & $\text{DA-MNIST}$ & $\lowercase{a}\text{MNIST-5}$ \\
% \midrule
% Vanilla     & 99.31 & 99.54 & 99.75  \\
% Dropout     & 99.38 & 99.56 & 99.74   \\
% \midrule
% SGHMC       & 99.55 & 99.71 & 99.77   \\
% \textbf{SGHMC-SA}    & \textbf{99.60} & \textbf{99.75} & \textbf{99.79}  \\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \vspace{-1em}
% \end{table}

% \begin{table}[t]
% \caption{Classification accuracy on FMNIST}
% \label{data-table2}
% \begin{center}
% \begin{small}
% \begin{sc}
% \label{tab:classi2}
% \begin{tabular}{lccc}
% \toprule
% Dataset & $\text{FMNIST}$ & $\text{DA-FMNIST}$ & $\lowercase{a}\text{FMNIST-5}$ \\
% \midrule
% Vanilla             & 92.73 & 93.14  &  94.48 \\
% Dropout             & 92.81 & 93.35  &  94.53 \\
% \midrule
% SGHMC               & 92.93 & 94.29  & 94.64  \\
% \textbf{SGHMC-SA}   & \textbf{93.01} & \textbf{94.38} & \textbf{94.78} \\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \vspace{-1em}
% \end{table}

\subsection{Defenses against Adversarial Attacks}
\label{adversarial}
Continuing with the setup in Sec. \ref{sec: mnist}, the third set of experiments focuses on evaluating model robustness. We apply the \textit{Fast Gradient Sign} method \citep{Goodfellow14a} to generate the adversarial examples with one single gradient step: 
\begin{equation}
\bm{x}_{adv} \leftarrow \bm{x}-\zeta \cdot \sign\{\delta_{\bm{x}} \max_{\y} \log \mathrm{P}(\y|\bm{x})\}, \nonumber
\end{equation}
where $\zeta$ ranges from $0.1, 0.2, \ldots, 0.5$ to control the different levels of  adversarial attacks.
% We expect less robust models perform considerably well on a certain dataset due to over-tuning; however, as the degree of adversarial attacks increases, the performance decreases sharply. In contrast, more robust models should be less affected by these adversarial attacks.

Similar to the setup in \citet{Li17}, we normalize the adversarial images by clipping to the range $[0, 1]$. In Fig. \ref{fig: adversarial}(b) and Fig.\ref{fig: adversarial}(d), we see no significant difference among all the four models in the early phase. As the degree of adversarial attacks arises, the images become vaguer as shown in Fig.\ref{fig: adversarial}(a) and Fig.\ref{fig: adversarial}(c). The performance of {Vanilla} decreases rapidly, reflecting its poor defense against adversarial attacks, while {Dropout} performs better than {Vanilla}. But {Dropout} is still significantly worse than the sampling based methods. The advantage of {SGHMC-SA} over {SGHMC} becomes more significant when $\zeta>0.25$. In the case of $\zeta=0.5$ in MNIST where the images are hardly recognizable, both {Vanilla} and {Dropout} models fail to identify the right images and their predictions are as worse as random guesses. However, {SGHMC-SA} model achieves roughly {11\%} higher than these two models and {1\%} higher than {SGHMC}, which demonstrates the robustness of  {SGHMC-SA}.

% Regarding the running time used, 100 epochs of the traditional training (Vanilla and Dropout) costs us 12.3 minutes, 100 epochs of \textbf{EP} training takes 32.3 minutes, as a contrast, 100 epochs of \textbf{sSGHMC} (90 epochs of ESM point estimation and 10 epochs of SGHMC) only spend 13.5 minutes using GPU Tesla P100, which showed our speed advantage over $\alpha$-divergence minimization.

% \begin{figure}
% \begin{subfigure}{0.17\linewidth}
% \includegraphics[scale=0.34]{figures/MNIST.PNG}
% \caption{$\zeta=..., 0.3, ...$.}
% \label{fig: 3a}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.3\linewidth}
% \includegraphics[scale=0.42]{figures/adversarial_comparison.pdf}
% \caption{MNIST}
% \label{fig: 3b}
% \end{subfigure}
% \hspace{0.5em}
% \begin{subfigure}{0.17\linewidth}
% \includegraphics[scale=0.34]{figures/fmnist.PNG}
% \caption{$\zeta=..., 0.3, ...$.}
% \label{fig: 3c}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.3\linewidth}
% \includegraphics[scale=0.42]{figures/adversarial_comparison_fmnist.pdf}
% \caption{F-MNIST}
% \label{fig: 3d}
% \end{subfigure}
% \caption{Adversarial test accuracies based on adversarial images of different levels}
% \vspace{-1.5em}
% \end{figure}

\begin{figure*}[!ht]
  \centering
  \subfigure[$\zeta=...$.]{\includegraphics[scale=0.3]{figures/MNIST.PNG}}\label{fig: 3a}
  \subfigure[MNIST]{\includegraphics[scale=0.35]{figures/adversarial_comparison.pdf}}\label{fig: 3b}\qquad
  \subfigure[$\zeta=...$.]{\includegraphics[scale=0.3]{figures/fmnist.PNG}}\label{fig: 3c}
  \subfigure[FMNIST]{\includegraphics[scale=0.35]{figures/adversarial_comparison_fmnist.pdf}}\label{fig: 3d}
  \caption{Adversarial test accuracies based on adversarial images of different levels}
  \label{fig: adversarial}
  \vspace{-1.5em}
\end{figure*}

% \begin{figure*}[!ht]
%   \centering
%   \subfigure[$\zeta=..., 0.3, ...$.]{\includegraphics[scale=0.34]{figures/MNIST.PNG}\label{fig: 3a}\qquad\qquad
%   \subfigure[MNIST]{\includegraphics[scale=0.42]{figures/adversarial_comparison.pdf}}\label{fig: 3b}\qquad\qquad
%   \subfigure[$\zeta=..., 0.3, ...$.]{\includegraphics[scale=0.34]{figures/fmnist.PNG}\label{fig: 3c}\qquad\qquad
%   \subfigure[FMNIST]{\includegraphics[scale=0.42]{figures/adversarial_comparison_fmnist.pdf}}\label{fig: 3d}\qquad\qquad
%   \caption{Adversarial test accuracies based on adversarial images of different levels}
% \end{figure*}


% \begin{figure}
%   \includegraphics[width=80mm,scale=0.5]{figures/adversarial_progressing.PNG}
%   \caption{Un-targeted attack: classification accuracy results based on various stepsizes}
%   \label{fig:architecture}
% \end{figure}

% \subsection{Unknown Target Test}

% Inspired by \citet{Gal16b}, besides the capability of knowing what a model knows, it is also interesting and important to make a deep model admit what it doesn't know. An intuitive strategy to access such abilities in point estimation is to set different thresholds, for example, if the threshold $\rho$ is 0.1, which means the output probability being higher than 0.6 is a cat, the one being lower than 0.4 is a dog, otherwise we leave the prediction undecided. Precision and recall are used to quantify such abilities, as shown in Figure 4, we can see setting $\rho=0.15$ gives us the best F1 score 72.3\% for \textbf{Vanilla}. 

% As a comparison, the other models use another strategy: namely if a classifier gives an 80\% credit interval containing 0.5, this corresponds to an unconfident input, otherwise, it makes a cat or dog decision (Figure. 5). 1500 images are tested including 500 dogs, 500 cats (the rest images in Kaggle) and 500 images of ostriches, elephants, wolves, ..., and pandas \citep{Deng09}. Suppose the model made 1200 decisions of which 900 are correct, then the model precision is 900/1200=75\%, its recall is 900/1000=90\%. The $F_1$ score is calculated as a comprehensive evaluation. Detailed experiments are implemented using the second DNN model mentioned before. As we can see from Table 3, the best \textbf{Vanilla} model (increasing accuracy by sacrificing recall) still fails to outperform the rest of the algorithms. \textbf{EP} gives better accuracy and F1 score than \textbf{Dropout}, but fails in recall, $\textbf{sSGHMC}$ demonstrated its overall advantage over these methods.




% % \begin{figure}
% %   \includegraphics[width=80mm,scale=0.5]{figures/known_target.PNG}
% %   \caption{Ostrich uncertainty test from cat \& dog classifier}
% %   \label{fig:architecture}
% % \end{figure}

% \begin{table}[t]
% \caption{Precision and recall rate of Cat \& Dog classifier from unknown animals}
% \label{unkownanimal-table}
% \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{lcccr}
% \toprule
%  & Vanilla & Dropout & EP & $\textbf{sSGHMC}$ \\
%     & $\rho=0.15$   &  $\alpha=0$          & $\alpha=1$ & $\eta=2e^{-7}$ \\
% \midrule
% Accuracy & 66.1\% & 62.4\% & 64.5\%   & \textbf{66.3\%} \\
% Recall   & 79.9\% & 87.5\% & 85.8\%   & 87.4\% \\
% F1-score  & 72.3\% & 72.8\% & 73.6\% & \textbf{75.4\%} \\

% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table}

% \begin{figure}[!ht]
% \begin{center}
%   \includegraphics[width=60mm,scale=0.5]{figures/unknown_target_vanilla.PNG}
%   \caption{Vanilla performance under different thresholds}
%   \label{fig:vanilla}
% \end{center}
% \end{figure}

% \begin{figure}[!ht]
% \begin{center}
%   \includegraphics[width=70mm,scale=0.5]{figures/unknown_label_ostrich.PNG}
%   \caption{Ostrich uncertainty test from cat \& dog classifier}
%   \label{fig:ostrich}
% \end{center}
% \end{figure}

% \begin{table}[t]
% \caption{Unknown targets test based on cat/dog classifier}
% \label{sample-table}
% \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{lcccr}
% \toprule
% Dataset & $\alpha=0$ & Gibbs-SGHMC & \textbf{sSGHMC} \\
%          &            & $\tau=1e-8$ & $\tau=6e-8$ \\
%          &            & waiting for check &  \\
% \midrule
% cat    & 75 & \textbf{92?} & 88 \\
% dog & 81 & 83 & 75 \\
% \textbf{Avg} & 78 & \textbf{83} & 81.5 \\
% \midrule
% ostrich    & 18 & 13 & \textbf{27} \\
% flamingo    & 15 & 17 & \textbf{18} \\
% wolf    & \textbf{24} & 15 & 22 \\
% fox    & 22 & 18 & \textbf{26} \\
% tiger    & \textbf{29} & 20 & 21 \\
% elephant    & 21 & 14 & 21 \\
% panda    & 19 & 19 & \textbf{31} \\
% plane    & 33 & 26 & \textbf{38} \\

% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table}


% \begin{table}[t]
% \caption{Precision and recall rate of Cat \& Dog classifier from unknown animals}
% \label{sample-table}
% \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{lcccr}
% \toprule
%   & $\alpha=0$ & Gibbs-SGHMC & SGHMC SA \\
%          &            & $\tau=1e-8$ & $\tau=6e-8$ \\
% \midrule
% Accuracy   & 63.1 & 64.8   & \textbf{65.3} \\
% Recall     & 78.0 & \textbf{87.5}   & 81.5 \\
% F1-score   & 69.7 & \textbf{74.4} & 72.5 \\

% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table}

\subsection{Residual Network Compression}

Our compression experiments are conducted on the CIFAR-10 dataset \citep{Alex09} with DA. SGHMC and the non-adaptive SGHMC-EM are chosen as baselines. Simulated annealing is used to enhance the non-convex optimization and the methods with simulated annealing are referred to as A-SGHMC, A-SGHMC-EM and A-SGHMC-SA, respectively. We report the best point estimate.
% \footnote{Since we are using the factor $N/n$ from Eq.(\ref{factor}), 0.002 comes from $0.1\times \frac{50,000}{1,000}$}

We first use SGHMC to train a Resnet20 model and apply the magnitude-based criterion to prune weights to all convolutional layers (except the very first one). All the following methods are evaluated based on the same setup except for different step sizes to learn the latent variables. 
% The step size is $\omega^{(k)}=0.02\times (k+1000)^{-0.75}$ for A-SGHMC-SA, $\omega^{(k)}\equiv 1$ for A-SGHMC-EM and $\omega^{(k)}\equiv 0$ for A-SGHMC. 
The sparse training takes 1000 epochs. The mini-batch size is 1000. The learning rate starts from 2e-9 \footnote[2]{It is equivalent to setting the learning rate to 1e-4 when we don't multiply the likelihood with $\frac{N}{n}$.} and is divided by 10 at the 700th and 900th epoch. We set the inverse temperature $\tau$ to 1000 and multiply $\tau$ by 1.005 every epoch . We fix $\nu=1000$ and $\lambda=1000$ for the inverse gamma prior. $v_0$ and $v_1$ are tuned based on different sparsity to maximize the performance. The smooth increase of the sparse rate follows the pruning rule in Algorithm \ref{alg: SGLD-EM}, and $\mathbb{D}$ and $\mathbb{f}$ are set to $0.99$ and $50$, respectively. The increase in the sparse rate $s$ is faster in the beginning and slower in the later phase to avoid destroying the network structure. Weight decay in the non-sparse layers $\mathcal{C}$ is set as 25. %To demonstrate the advantage of the self-adapting penalty functions over the others, we compare a list of fixed $L_1$ penalties and $L_2$ penalties to the sparse layers $\mathcal{X}$ to show the strength of our proposed method.
%mitigate the potential problem of local traps\footnote{To accommodate for the standard settings in training Resnet with crossentropy loss, we ignore the factor $N/n$ from Eq.(\ref{factor}), it is equivalent to set $\tau=2\times10^4$ in Eq.(\ref{factor})}.
\begin{table}[t]
\caption{Resnet20 Compression on CIFAR10. When $\mathbb{S}=0.9$, we fix $v_0=0.005$, $v_1=$1e-5; When $\mathbb{S}=0.7$, we fix $v_0=0.1$, $v_1=$5e-5; When $\mathbb{S}=0.5$, we fix $v_0=0.1$, $v_1=$5e-4; When $\mathbb{S}=0.3$, we fix $v_0=0.5$, $v_1=$1e-3.}
\label{compression_1}
\begin{center}
\begin{small}
% \scriptsize
\begin{sc}
% \begin{tabular}{lccccc}
\begin{tabularx}{0.55\textwidth}{ccccc}
\toprule
 Methods $\backslash\ $ $\ \mathbb{S}$ & $30\%$ & $50\%$ & $70\%$ & $90\%$ \\
\midrule
% $L_1=1\times10^{-4}$   &  \textbf{94.09}  & \textbf{93.74}   & 92.98   & 89.47 \\
% % $L_1=3\times10^{-4}$   &  94.03  & 93.68   & \textbf{93.01}   & 89.62 \\
% % $L_1=1\times10^{-3}$   &  92.88   &  92.75  &  92.62  & 89.95 \\
% $L_1=3\times10^{-3}$   &  92.48  &  92.49  &  92.10  & \textbf{91.12} \\
% % $L_1=1\times10^{-2}$   &  89.50  &  89.79  &  90.07  & 89.83 \\
% % $L_1=3\times10^{-2}$   &  83.02  &  82.36  &  82.88  & 83.50 \\
% \midrule
% % $L_2=1\times10^{-4}$   & 94.15  &  93.78  &  93.12  & 89.37 \\
% % $L_2=1\times10^{-3}$   & 94.03  &  93.64  &  93.06  & 89.29 \\
% % $L_2=1\times10^{-2}$   & 94.17  & 93.82   &  93.17  & 90.11 \\
% $L_2=3\times10^{-2}$   & \textbf{94.20}  & \textbf{93.99}   &  93.37  & 91.15 \\
% $L_2=1\times10^{-1}$   &  94.02  &  93.96  &  \textbf{93.50}  & 91.20 \\
% $L_2=3\times10^{-1}$   &  93.72  &  93.57  &  93.37  & \textbf{91.27} \\
% $L_2=6\times10^{-1}$   &  93.30  &  93.09  &  93.00  & 91.40 \\
% $L_2=1\times10^{0}$   &  92.94  & 92.90   &  92.56  & 91.16 \\
% \midrule
% \textbf{SGHMC-SSG}    & \textbf{94.27}  &  93.94  &  \textbf{93.63}  &  \textbf{91.51} \\
A-SGHMC  &  94.07  & 94.16   &  93.16  & 90.59 \\
A-SGHMC-EM   &  94.18  & 94.19   &  93.41  & 91.26 \\
SGHMC-SA    & {94.13}  &  {94.11}  &  {93.52}  &  {91.45} \\
\textbf{A-SGHMC-SA}    & \textbf{94.23}  &  \textbf{94.27}  &  \textbf{93.74}  &  \textbf{91.68} \\
\bottomrule
\end{tabularx}
\end{sc}
\end{small}
\end{center}
\vspace{-1em}
\end{table}

As shown in Table \ref{compression_1}, A-SGHMC-SA doesn't distinguish itself from A-SGHMC-EM and A-SGHMC when the sparse rate $\mathbb{S}$ is small, but outperforms the baselines given a large sparse rate.
%all the other methods based on fixed $L_1$ and $L_2$ penalties.
The pretrained model has accuracy 93.90\%, however,the prediction performance can be improved to the state-of-the-art $94.27\%$ with 50\% sparsity. Most notably, we obtain 91.68\% accuracy based on 27K parameters (90\% sparsity) in Resnet20. By contrast, targeted dropout obtained 91.48\% accuracy based on 47K parameters (90\% sparsity) of Resnet32 \citep{Aidan18}, BC-GHS achieves 91.0\% accuracy based on 8M parameters (94.5\% sparsity) of VGG models \citep{Louizos17}. We also notice that when simulated annealing is not used as in SGHMC-SA, the performance will decrease by 0.2\% to 0.3\%. When we use batch size 2000 and inverse temperature schedule $\tau^{(k)}=20\times 1.01^k$, A-SGHMC-SA still achieves roughly the same level, but the prediction of SGHMC-SA can be 1\% lower than A-SGHMC-SA. 

%As the sparse rate increases, a larger regularization is needed to yield a satisfying performance.

==> NIPS 2019 An Adaptive Empirical Bayesian Method for Sparse Deep Learning -arXiv/intro.tex <==
%Deep learning has achieved many successes in various areas. However, researchers have largely focused on increasing its learning ability by merely applying point estimation without considering uncertainty quantification. As discussed by \citet{Kendall17, Gal17,Amodei16}, the AI safety problems can never be ignored: Reported by US News, an image classification system confused humans with gorillas; A blog article by Keras developers showed a well-trained ImageNet model predicted adversarial sea snake images as magpies with 99.99\% confidence; Several serious traffic fatalities caused by autonomous cars were reported recently, resulting from the intelligent systems for assisted driving failing to recognize objects. These issues, which weakened the reliability of point estimation in deep learning, can be considerably alleviated given a better uncertainty quantification of the decisions.

%%%
% A brief intro of bayesian deep learning and SG-MCMC
%%%
% Bayesian deep learning, which evolved from Bayesian neural networks \citep{Neal96,Denker90}, provides an alternative to point estimation due to its close connection to both Bayesian probability theory and cutting-edge deep learning models. Its merit of quantifing uncertainty has been studied \citep{Gal16b}, which not only increases the predictive power of deep neural networks (DNNs) but also further provides a more robust estimation to enhance AI safety. 

MCMC, known for its asymptotic properties, has not been fully investigated in deep neural networks (DNNs) due to its unscalability in dealing with big data. Stochastic gradient Langevin dynamics (SGLD) \citep{Welling11}, the first stochastic gradient MCMC (SG-MCMC) algorithm, tackled this issue by adding noise to the stochastic gradient, smoothing the transition between optimization and sampling and making MCMC scalable. \citet{Chen14} proposed using stochastic gradient Hamiltonian Monte Carlo (SGHMC), the second-order SG-MCMC, which was shown to converge faster. In addition to modeling uncertainty, SG-MCMC also has remarkable non-convex optimization abilities. \citet{Maxim17,Xu18} proved that SGLD, the first-order SG-MCMC, is guaranteed to converge to an approximate global minimum of the empirical risk in finite time. \citet{Yuchen17} showed that SGLD hits the approximate local minimum of the population risk in polynomial time. \citet{Mangoubi18} further demonstrated SGLD with simulated annealing has a higher chance to obtain the global minima on a wider class of non-convex functions. However, all the analyses fail when DNN has too many parameters, and %compared to the amount of data. %One main reason that causes that over-fitting problem is the over-specified models. 
% When this happens, 
the over-specified model tends to have a large prediction variance, resulting in poor generalization and causing over-fitting. Therefore, a proper model selection is on demand at this situation.% \citep{Chen15}. % \citet{Saatci17} used SGHMC with GANs \citep{Goodfellow14b} to achieve a fully probabilistic inference and showed the Bayesian GAN model with only 100 labeled images was able to achieve 99.3\% testing accuracy in MNIST dataset. 
%Considering the pathological curvature that causes the SGLD methods inefficient in DNN models, \citet{Li16} proposed combining adaptive preconditioners with SGLD (pSGLD) to adapt to the local geometry and obtained state-of-the-art performance on MNIST dataset. 
%Particularly, \citet{Gal16a,Gal16b} described dropout  \citep{Srivastava14} as a variational Bayesian approximation. Through enabling dropout in the testing period, the randomly dropped neurons generate some amount of uncertainty with almost no added cost. However, the dropout Bayesian approximation is variational inference (VI) based thus it is vulnerable to underestimating uncertainty. %In addition, due to the inefficiency of sampling from complex posterior, applications of Bayesian deep learning models were still largely limited. 

%In addition, \citet{Gal17} connected Bayesian Convolutional Neural Networks (BCNNs) \citep{Gal16a} with active learning \citep{Cohn96} and were able to achieve 1.64\% test error on MNIST with only 1000 labeled images.

% To tackle this drawback, various approximations have been proposed. \citet{Blundell15} proposed a variational inference (VI) method: \textit{Bayes by Backprop}, by doubling the number of model parameters. Its performance is comparable to dropout but the training is slow. 

% \citet{Li17} mitigate that problem by generalizing the framework to the black-box $\alpha$-divergence minimization, where both expectation propagation (EP) and variational inference (VI) were employed. By increasing the value of $\alpha$ from 0 to 1, the inference gradually evolves from VI to EP, thus an improvement on uncertainty quantification is achieved with the sacrifice of the performance of the point estimation. Additionally, a sufficient number of forward passes is required in training, which makes a reasonable running time unattainable. 

% The increasing concern for AI safety problems brings back our attention to Markov Chain Monte Carlo (MCMC), [which in deep learning has not been fully investigated due to its unscalability on big data and large models]->[why MCMC is better]. 


%%%
% Merits of SG-MCMC, and its weakness when meeting DNN
%%%
% In addition to modeling uncertainty, SG-MCMC also has remarkable non-convex optimization abilities. \citet{Maxim17,Xu18} proved that SGLD, the first-order SG-MCMC, is guaranteed to converge to an approximate global minimum of the empirical risk in finite time. \citet{Yuchen17} showed that SGLD has a considerable chance to hit the approximate local minimum of the population risk in polynomial time and escape “shallow” local minima that only exist in the empirical risk. "\citet{Mangoubi18} further analyzed that SGLD with simulated annealing has a higher chance to hit the global minima than SGLD on a wider class of non-convex functions". However, all the analyses fail when DNN has too many parameters, and %compared to the amount of data. %One main reason that causes that over-fitting problem is the over-specified models. 
% % When this happens, 
% the over-specified model tends to have a large prediction variance, resulting in poor generalization and causing over-fitting. Therefore, a proper model selection is on demand at this situation.%will be powerful to alleviate over-fitting.
% %, given a smooth enough objective function and an appropriate temperature

%%%
% An intro of model selection method
%%%
A standard method to deal with model selection is variable selection. Notably, the best variable selection based on the $L_0$ penalty is conceptually ideal for sparsity detection but is computationally slow. Two alternatives emerged to approximate it. On the one hand, penalized likelihood approaches, such as Lasso \citep{Tibshirani94}, induce sparsity due to the geometry that underlies the $L_1$ penalty. To better handle highly correlated variables, Elastic Net was proposed \citep{Zou05} and makes a compromise between $L_1$ penalty and $L_2$ penalty. On the other hand, spike-and-slab approaches to Bayesian variable selection originates from probabilistic considerations. \citet{George93} proposed to build a continuous approximation of the spike-and-slab prior to sample from a hierarchical Bayesian model using Gibbs sampling. This continuous relaxation inspired the efficient EM variable selection (EMVS) algorithm in linear models \citep{Rockova14, Rockova18}. %A similar algorithm \citep{Rockova18} using Spike-and-slab LASSO (SSL) priors is presented later to bridge the gap between variable selection and penalized likelihood estimation. 

%%%
% Advances of model selection in DNN
%%%
Despite the advances of model selection in linear systems, model selection in DNNs has received less attention. %A few attempts worked well on shallow Bayesian neural networks (BNNs): \citet{liang_vs_2018} % proposed to use parallel MCMC \citep{song14} to sample from BNNs with Gaussian priors on the weights and
%analyzed the consistency properties of variable selection using Gaussian priors on BNNs. 
\citet{Ghosh18} proposed to use variational inference (VI) based on regularized horseshoe priors to obtain a compact model. \citet{liang_vs_2018} presented the theory of posterior consistency for Bayesian neural networks (BNNs) with Gaussian priors, and \citet{ye18} applied a greedy elimination algorithm to conduct group model selection with the group Lasso penalty. Although these works only show the performance of shallow BNNs, the experimental methodologies imply the potential of model selection in DNNs. 
\citet{Louizos17} studied scale mixtures of Gaussian priors and half-Cauchy scale priors for the hidden units of VGG models \citep{Karen14} 
and achieved good model compression performance on CIFAR10 \citep{Alex09} using VI. However, due to the limitation of VI in non-convex optimization, the compression is still not sparse enough and can be further optimized.  %Variable selection in much more complex DNNs is still an open question.%\citep{Aidan18} proposed the targeted dropout method to rank weights or units according to the magnitude and prune the elements with low importance. %They achieved xx\% on CIFAR10 using Resnet32. 
% the proven success of $L_1$ penalty in variable selection, and the wide application of $L_2$ penalty in DNNs


%%%
% Our method, to apply model selection in DNN
%%%
%which is impractical in real applications for smart devices.
Over-parameterized DNNs often demand for tremendous memory use and heavy computational resources, which is impractical for smart devices. More critically, over-parametrization frequently overfits the data and results in worse performance \citep{lin17}. To ensure the efficiency of the sparse sampling algorithm without over-shrinkage in DNN models, we propose an AEB method to adaptively sample from a hierarchical Bayesian DNN model with spike-and-slab Gaussian-Laplace (SSGL) priors and the priors are learned through optimization instead of sampling. The AEB method differs from the full Bayesian method in that the priors are inferred from the empirical data and the uncertainty of the priors is no longer considered to speed up the inference. In order to optimize the latent variables without affecting the convergence to the asymptotically correct distribution, stochastic approximation (SA) \citep{Albert90}, a standard method for adaptive sampling \citep{andrieu05, Liang10}, naturally fits to train the adaptive hierarchical Bayesian model. %As a result, the asymptotic property allows us to combine simulated annealing to obtain a better point estimate in non-convex optimization.
%EM is an efficient algorithm to deal with this type of priors in linear models with closed-form update. Unfortunately, EM is known to be sensitive to hyperparameters, vulnerable to local traps \citet{ma18}, and unable to .  
%showed theoretically EM can be quite slow in searching global minima in Gaussian mixture models given bad initializations. 
%To tackle this issue, our solution is to use 
%\citet{Rockova17} alleviates the local entrapment problem by deploying an ensemble of interactive repulsive particles. 

% Motivated by the computational efficiency of the EM algorithm \citep{Dempster77}, the proven success of $L_1$ penalty in variable selection, and the wide application of $L_2$ penalty (known as weight decay in DNNs) in parameter estimation, 

%%%
% List our contributions
%%%
In this paper, we propose a sparse Bayesian deep learning algorithm, SG-MCMC-SA, to adaptively learn the hierarchical Bayes mixture models in DNNs. This algorithm has four main contributions: 
\begin{itemize}
\item We propose a novel AEB method to efficiently train hierarchical Bayesian mixture DNN models, where the parameters are learned through sampling while the priors are learned through optimization.

\item We prove the convergence of this approach to the asymptotically correct distribution, and it can be further generalized to a class of adaptive sampling algorithms for estimating state-space models in deep learning.

\item We apply this adaptive sampling algorithm in the DNN compression problems firstly, with potential extension to a variety of model compression problems.
% \item By automatically searching the over-fitted parameter space to add more penalties, the proposed method quantifies the posterior distributions of the decisive variables more accurately;
% \item Empirically, the algorithm demonstrates more resistance to over-fitting in simulations, leads to the state-of-the-art performance on MNIST and Fashion-MNIST and shows more robustness over SG-MCMC.
\item It achieves the state of the art in terms of compression rates, which is 91.68\% accuracy on CIFAR10 using only 27K parameters (90\% sparsity) with Resnet20  \citep{kaiming15}.%, which outperforms the existing methods by a large margin.
\end{itemize}

==> NIPS 2019 An Adaptive Empirical Bayesian Method for Sparse Deep Learning -arXiv/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

\DeclareMathOperator{\V}{\mathbb{V}}
\DeclareMathOperator*{\where}{where}
\DeclareMathOperator*{\for}{for}
\DeclareMathOperator*{\sufficiently}{sufficiently}
\DeclareMathOperator*{\larges}{large}
\DeclareMathOperator*{\any}{any}
\DeclareMathOperator*{\using}{using}
\DeclareMathOperator*{\as}{as}
\DeclareMathOperator*{\Claim}{Claim}
\DeclareMathOperator*{\Proposition}{Proposition}
\DeclareMathOperator*{\x}{x}
\DeclareMathOperator*{\y}{y}
\DeclareMathOperator*{\w}{w}
\DeclareMathOperator*{\MLE}{MLE}
\DeclareMathOperator*{\MAP}{MAP}
\DeclareMathOperator*{\diag}{diag}
% \DeclareMathOperator*{\sign}{sign}
\DeclareMathOperator*{\Inv}{Inv}
\DeclareMathOperator*{\sSGHMC}{sSGHMC}
\DeclareMathOperator*{\esSGHMC}{esSGHMC}
\DeclareMathOperator*{\heng}{-}
\DeclareMathOperator*{\stopol}{Stochastic\ Pooling}
\DeclareMathOperator*{\randfilters}{Random\ Filters}
\newcommand\norm[1]{\left\lVert#1\right\rVert}

\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{assumption}{Assumption}

\let\origtheassumption\theassumption

\edef\oldassumption{\the\numexpr\value{assumption}+1}

% \newcommand{\theHalgorithm}{\arabic{algorithm}}


==> NIPS 2019 An Adaptive Empirical Bayesian Method for Sparse Deep Learning -arXiv/relworks.tex <==
% \begin{corollary}
% Given fixed stepsize $\epsilon$, the distribution of $\bm{\beta}^{(k)}$ from SG-MCMC-SA converges weakly to the invariant distribution $\pi(\bm{\beta}, \bm{\rho}^{*}, \bm{\kappa}^{*}, \delta^*|\mathcal{D})$ with rate $\alpha\in (0, 1]$ as $\epsilon\rightarrow 0$.
% \end{corollary}


% \citet{Teh14,Chen15} also pointed out that SGHMC has an optimal stepsize $\epsilon \propto K^{-1/3}$ with respect to the bias of the expected sample average and $\epsilon \propto K^{-1/5}$ with respect to MSE in the $K$-th iteration. When considering the practical issue of limited time, since the polynomial-decay learning rate decreases very fast in the early phase, it can potentially influence the efficiency. To overcome that issue, \citet{Welling11} kept a constant stepsize once the stepsize decreased below a critical level; \citet{Chen14} used a small fixed $\epsilon$ to gain efficiency. We instead seek a balance between fixed value and polynomial decay and use an exponential decay $(1-0.001)^K$ to mildly decrease the stepsize in the early phase.

% In addition, in Hamiltonian dynamics, given injected noise variance $M$, the kinetic energy is usually defined as $K(p)=p^TM^{-1}p/2$ \citep{Neal10}, whereas in the backprop based DNN, we found that $K(p)=p^Tp/2$ achieves a much faster mixing without violating the reversibility and conservation. The proof is similar to \citet{Neal10} and is omitted in this paper. This leads to a modification of SGHMC from letting $v\sim \mathcal{N}(0, \epsilon I)$, $\Delta v=-\epsilon^2M^{-1}\Delta U(\delta)-\epsilon M^{-1}Cv +\mathcal{N}(0, 2\epsilon^3M^{-1}(C-\hat B)M^{-1})$ to the following equation
% \begin{equation}
% \begin{split}
% &letting\ v\sim \mathcal{N}(0, \epsilon V_l) \\
% &\Delta\delta = v \\
% &\Delta v=-\epsilon^2\Delta U(\delta)-\epsilon Cv +\mathcal{N}(0, 2\epsilon^3(C-\hat B)).
% \end{split}
% \end{equation}

% In our model, $V_l$ is estimated from empirical Fisher information $V_l=\dfrac{\sum_{k=1}^{p_l} (\pi_{\beta_{(t)}}-\bar\pi_{\beta_{(t)}})^2}{p_l-1}$  for each layer $l$\ \citep{Ahn12}. In the sparse weights, to account for the different variances for different weights, we can modify $V_l$ to be $V_l=E(\Sigma_l)$, where $E_{\beta_j}(\Sigma_l)=(\sigma^*)^2 [v_0 (1-p_j^*) + v_1 p_j^*]$. If we further assume $\alpha=\epsilon C$, $\eta=\epsilon^2$, $b=\epsilon \hat B$, the implementation details are shown in Algorithm 1. We refer to the SGHMC pretrained with ESM framework as \textbf{sSGHMC}.
Dropout alleviates over-fitting and provides an efficient way of making bagging practical for ensembles of countless sub-networks. It can be interpreted as assigning mixture priors on the hidden units \citep{Yarin16b}.
From the Bayesian perspective, our proposed algorithm differs from Dropout and its variants in treating the priors: our algorithm keeps updating the priors during posterior inference, rather than keep them fixed. The inclusion of scaled mixture priors in deep learning models were also studied in \citet{Blundell15,Li16} with encouraging results. 

Our algorithm shares some similarities with variational Bayes (VB) and EMVS, such as the efficiency and the lower bound approximation, but differs from them 
fundamentally. First, our proposed algorithm only approximates the latent variables, while sampling the weights via SG-MCMC. Second, EMVS, mainly designed for linear models with closed-form update, doesn't work for highly non-linear DNN models lacking closed-form solution. In addition, it is unable to optimize the latent variables stochastically. A trivial implementation of EMVS in DNNs will likely cause the latent variables to trap in poor local optima.

Our setup differs from Bayesian Elastic Net \citep{li2010, hans11} and mixed shrinkage prior \citep{Georgios14} in that our model not only is self-adaptive but also yields a more efficient framework for inference.

%The use of numerical differentiation implicitly allows the pruned values to be able to change their value if they become important again. %Due to the rapid development of automatic differentiation, we are not concerned with the problem when the weights $\bm{\beta}$ are mathematically not differentiable at 0.


% Inspired by MCMC model composition ($MC^3$) by \citet{Madigan94}, the presence of model uncertainty enables us to achieve better performance in point estimation through BMA \citep{Welling11,Li16} from MCMC samples. If we simulate Markov Chain $\beta(t), t=1,2,\ldots, N$ from invariant distribution $\pi(\beta^{(k)}|\mathcal{D})$, then the weigted average (Welling, M., 2011) $\dfrac{\sum_{t=1}^{N} \epsilon^{(k)} \psi(\beta^{(k)})}{\sum_{t=1}^{N}\epsilon^{(k)}}$ converges to  $E[\psi(\hat \beta)]$ as $N \rightarrow \infty$. we refer to \textbf{sSGHMC} with BMA as \textbf{esSGHMC}. 

% \begin{algorithm}[tb]
%    \caption{Posterior Sampling with spike-and-slab prior: $\epsilon$ is the stepsize, $\eta=\epsilon^2$ is the learning rate, $\alpha$ corresponds to the friction term, $p_l$ is the number of parameters in layer $l$, $\pi_{\beta}$ is the posterior derivative with respect to $\beta$. In practice, $\alpha=0.01$, $b=\dfrac{1}{2}\eta$, $\kappa=0.001$, L=5}
% \begin{algorithmic}
%    \Require{mini-batch $\mathcal{D}$}
%    \State{Initialize $\beta$, $\sigma$ and $p$ from scratch or ESM}
%    \For{$K$ in $1, 2, ..., m$}
%    \State{$\epsilon \leftarrow \epsilon-\kappa \epsilon$; $\eta\leftarrow\epsilon^2$}
%    \For{each layer $l$}
%    \If{weights are sparse}
%    \State{$V_l=E_{\beta}(\Sigma_l)$}
%    \Else
%    \State{$V_l=\dfrac{\sum_{k=1}^{p_l} (\pi_{\beta_{(t)}}-\bar\pi_{\beta_{(t)}})^2}{p_l-1}$}
%    \EndIf
%    \State{Sample $v \sim \epsilon \mathcal{N}(0, V_l)$}
%    \For{each leapfrog $1, 2, \ldots, L$}
%    \State{$\beta \leftarrow \beta + v$}
%    \State{$v \leftarrow (1-\alpha) v - \eta \pi_{\beta}(\beta, \sigma^*, \gamma|\mathcal{D}) + 2(\alpha-b)\eta\mathcal{N}(0, V_l)$}
%    \EndFor
%    \EndFor
%    \State{Append $\beta$ to the chains}
%    \EndFor
% \end{algorithmic}
% \end{algorithm}

% \subsection{Comparison with DropConnect}

% Binary DropConnect \citep{Liwan13} and our proposed algorithm both assume the spike-and-slab prior on the weights. The difference is that the former doesn't update the prior parameters during inference while the later one does.

==> NIPS 2019 An Adaptive Empirical Bayesian Method for Sparse Deep Learning -arXiv/sa.tex <==
% original words: it prevents the network weights from collaborating with one another to memorize the training examples; DropConnect which generalizes Dropout by randomly dropping the weights rather than the activations; MNIST:  DropConnect is even slower to converge than Dropout, but yields a lower test error in the end. fmnist: DropConnect prevents overfitting of the fully connected layer better than Dropout in this experiment; DropConnect, which generalizes Hinton et al. ’s Dropout (Hinton et al., 2012) to the entire connectivity structure of a fully connected neural network layer. 

%  Similarly, binary DropConnect can be viewed as using the Spike-and-Slab prior on the weights without updating the prior parameters during inference

% Empirically, dropout is implemented in the layers where weights are highly fat-tailed, we may randomly ``drop'' the neurons to achieve better predictive performance. 
%Dropout randomly drops activations, which has the potential to destroy the connectivity structure of a fully connected neural network layer. \citet{Liwan13} fix that problem by proposing DropConnect to randomly drop the weights and achieve slightly better regularization on large neural networks. 
%


%However, to the best of our knowledge, none of the existing SG-MCMC methods could deal with complex posterior with latent variables. 
%EM algorithm \citep{Dempster77} naturally fits the scenario where the sparse priors need to be handled efficiently.
%Intuitively, the Bayesian formulation with model averaging and the spike-and-slab priors is expected to obtain better predictive performance through averages from a "selective" group of "good" submodels, rather than averaging exponentially many posterior probabilities roughly. For the rest of the weight priors and bias priors, we just assume they follow a certain Gaussian distribution.

% \begin{figure*}[!ht]
% \begin{center}  \includegraphics[scale=0.33]{figures/dropout_weight_uncertainty_v9.pdf}
%   \caption{Model Structure}
%   \label{Model Structure}
% \vspace{-1.5em}
% \end{center}
% \end{figure*}

% \subsection{A new formulation based on deep SSGL priors}
\subsection{A hierarchical formulation with deep SSGL priors}


% \begin{figure*}[t!]
%     \centering
%     \begin{subfigure}[t]{0.67\textwidth}
%         \centering
%         \includegraphics[scale=0.3]{figures/dropout_weight_uncertainty_v9.pdf}
%         \caption{Model Structure}
%     \end{subfigure}%
%     ~ 
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[scale=0.08]{figures/dropout.pdf}
%         \caption{Dropout}
%     \end{subfigure}
%     \caption{Left: each weight is a fixed value, neurons are randomly dropped, providing an approximation of $2^N$ possible models; Right: weights are assigned to specific distributions, which end up with several promising models}
% \end{figure*}

% \begin{figure*}[t!]
%     \centering 
%     \begin{subfigure}[t]{0.67\textwidth}
%         \centering
%         \includegraphics[scale=0.3]{figures/dropout_weight_uncertainty_v9.pdf}
%         \caption{Model Structure}
%     \end{subfigure}%
%     ~ 
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[scale=0.08]{figures/dropout.pdf}
%         \caption{Dropout}
%     \end{subfigure}
%     \caption{Left: each weight is a fixed value, neurons are randomly dropped, providing an approximation of $2^N$ possible models; Right: weights are assigned to specific distributions, which end up with several promising models}
% \end{figure*}


Inspired by the hierarchical Bayesian formulation for sparse inference \citep{George93}, we assume the weight $\bm{\beta}_{lj}$ in sparse layer $l$ with index $j$ follows the SSGL prior
\begin{equation}
\beta_{lj} | \sigma^2, \gamma_{lj} \sim (1-\gamma_{lj}) \mathcal{L}(0, \sigma v_0)+\gamma_{lj} \mathcal{N}(0, \sigma^2 v_1).
\end{equation}
% \begin{equation}
% \beta_{lj} | \sigma^2, \gamma_{lj} \propto \frac{1}{\sigma}\exp\left[{\frac{(1-\gamma_{lj})|\beta_{lj}|}{\sigma v_0} +\frac{\gamma_{lj}\beta_{lj}^2}{\sigma^2 v_1}}\right],
% \end{equation}
where $\gamma_{lj}\in \{0, 1\}$, $\bm{\beta}_l\in\mathbb{R}^{p_l}$,  $\sigma^2\in\mathbb{R}$, $\mathcal{L}(0, \sigma v_0)$ denotes a Laplace distribution with mean $0$ and scale $\sigma v_0$, and $\mathcal{N}(0, \sigma^2 v_1)$ denotes a Normal distribution with mean $0$ and variance $\sigma^2 v_1$. The sparse layer can be the fully connected layers (FC) in a shallow CNN or Convolutional layers in ResNet. If we have $\gamma_{lj}=0$, the prior behaves like Lasso, which leads to a shrinkage effect; when $\gamma_{lj}=1$, the $L_2$ penalty dominates. The likelihood follows
% http://web.engr.oregonstate.edu/~xfern/classes/cs534/notes/logistic-regression-note.pdf
\begin{equation}  
\label{eq:4}
\pi(\mathcal{B}|\bm{\beta},\sigma^2)=\left\{  
             \begin{array}{lr}  
             \dfrac{\exp\left\{-\dfrac{\sum_{i\in \mathcal{S}} (y_{i}-\psi(\bm{x}_{i};\bm{\beta}))^2}{2\sigma^2}\right\}}{(2\pi\sigma^2)^{n/2}} & \text{(regression)}, \\  
              & \\
%              \prod_{i=1}^{m} \psi(\bm{x_i};\bm{\beta})^{y_i} \left(1-\psi(x_i;\bm{\beta})\right)^{1-y_i}, &  \text{classification}  
             \prod\limits_{i\in \mathcal{S}} \dfrac{\exp\{\psi_{y_i}(\bm{x}_{i};\bm{\beta})\}}{\sum_{t=1}^K \exp\{\psi_{t}(\bm{x}_i;\bm{\beta})\}} & \text{(classification)}, 
             \end{array}
\right.  
\end{equation} 
where $\psi(\bm{x}_{i};\bm{\beta})$ is a linear or non-linear mapping, and $y_i \in \{1,2,\dots,K\}$ is the response value of the $i$-th example. In addition, the variance $\sigma^2$ follows an inverse gamma prior $\pi(\sigma^2)=IG(\nu/2, \nu\lambda/2)$.
The i.i.d. Bernoulli prior is used for $\bm{\gamma}$, namely $\pi(\bm{\gamma}_l|\delta_l) = \delta_l^{|\bm{\gamma}_l|} (1-\delta_l)^{p_l-|\bm{\gamma}_l|}$
where $\delta_l\in\mathbb{R}$ follows Beta distribution $\pi(\delta_l) \propto \delta_l^{a-1}(1-\delta_l)^{b-1}$. The use of self-adaptive penalty enables the model to learn the level of sparsity automatically. 
Finally, our posterior follows
\begin{equation}
\pi(\bm{\beta}, \sigma^2, \delta, \bm{\gamma}|\mathcal{B}) \propto \pi(\mathcal{B}|\bm{\beta}, \sigma^2)^{\frac{N}{n}} \pi(\bm{\beta}|\sigma^2,\bm{\gamma}) \pi(\sigma^2| \bm{\gamma}) \pi(\bm{\gamma}|\delta) \pi(\delta).
\end{equation}

% \begin{equation}  
% \label{eq:4}
% \pi(\mathcal{B}|\bm{\beta}, \sigma^2) = \prod\limits_{i\in \mathcal{S}} \dfrac{\exp\{\psi_{y_i}(\bm{x}_{i};\bm{\beta})\}}{\sum_{t=1}^K \exp\{\psi_{t}(\bm{x}_i;\bm{\beta})\}}
% \end{equation}

% \begin{equation}  
% \label{eq:4}
% \pi(\mathcal{B}|\bm{\beta}, \sigma^2) =\left\{  
%              \begin{array}{lr}  
%              (2\pi\sigma^2)^{-n/2}\exp\left\{-\dfrac{1}{2\sigma^2}\sum_{i\in \mathcal{S}} (y_{i}-\psi(\bm{x}_{i};\bm{\beta}))^2\right\} & \text{(regression)}   \\  
%               & \\
% %              \prod_{i=1}^{m} \psi(\bm{x_i};\bm{\beta})^{y_i} \left(1-\psi(x_i;\bm{\beta})\right)^{1-y_i}, &  \text{classification}  
%              \prod\limits_{i\in \mathcal{S}} \dfrac{\exp\{\psi_{y_i}(\bm{x}_{i};\bm{\beta})\}}{\sum_{t=1}^K \exp\{\psi_{t}(\bm{x}_i;\bm{\beta})\}} &  \text{(classification),}  
%              \end{array}  
% \right.  
% \end{equation} 

%, note that we use $\pi(\mathcal{B}|\bm{\beta}, \sigma^2)$ instead of $\pi(\mathcal{B}|\bm{\beta})$ for unification without effecting the result.





%The EMVS approach is efficient in identifying potential sparse high posterior probability submodels on high-dimensional regression \citep{Rockova14} and classification problem \citep{McDermott16}. These characteristics are helpful for large neural network computation, thus we refer to the stochastic version of the EMVS algorithm as Expectation Stochastic-Maximization (ESM).

\subsection{Empirical Bayesian with approximate priors}

To speed up the inference, we propose the AEB method by sampling $\bm{\beta}$ and optimizing $\sigma^2, \delta, \bm{\gamma}$, where uncertainty of the hyperparameters is not considered. Because the binary variable $\bm{\gamma}$ is harder to optimize directly, we consider optimizing the adaptive posterior $\E_{\bm{\gamma}|\cdot, \mathcal{D}}\left[\pi(\bm{\beta}, \sigma^2, \delta, \bm{\gamma}|\mathcal{D})\right]$ \footnote{$\E_{\bm{\gamma}|\cdot, \mathcal{D}}[\cdot]$ is short for $\E_{\bm{\gamma}|\beta^{(k)}, \sigma^{(k)},\delta^{(k)}, \mathcal{D}}[\cdot]$.} instead. Due to the limited memory, which restricts us from sampling directly from $\mathcal{D}$, we choose to sample $\bm{\beta}$ from $\E_{\bm{\gamma}|\cdot,\mathcal{D}}\left[\E_{\mathcal{B}}\left[\pi(\bm{\beta}, \sigma^2, \delta, \bm{\gamma}|\mathcal{B})\right]\right]$ \footnote{ $\E_{\mathcal{B}}[\pi(\bm{\beta}, \sigma^2, \delta, \bm{\gamma}|\mathcal{B})]$ denotes $\int_{\mathcal{D}}\pi(\bm{\beta}, \sigma^2, \delta, \bm{\gamma}|\mathcal{B})d\mathcal{B}$}. By Fubini's theorem and Jensen's inequality, we have
\begin{equation}
\begin{split}
\label{js_}
&\log \E_{\bm{\gamma}|\cdot,\mathcal{D}}\left[\E_{\mathcal{B}}\left[\pi(\bm{\beta}, \sigma^2, \delta, \bm{\gamma}|\mathcal{B})\right]\right]=\log \E_{\mathcal{B}}\left[\E_{\bm{\gamma}|\cdot,\mathcal{D}}\left[\pi(\bm{\beta}, \sigma^2, \delta, \bm{\gamma}|\mathcal{B})\right]\right]\\
\geq &\E_{\mathcal{B}}\left[\log  \E_{\bm{\gamma}|\cdot,\mathcal{D}}\left[\pi(\bm{\beta}, \sigma^2, \delta, \bm{\gamma}|\mathcal{B})\right]\right]\geq \E_{\mathcal{B}}\left[\E_{\bm{\gamma}|\cdot,\mathcal{D}}\left[\log\pi(\bm{\beta}, \sigma^2, \delta, \bm{\gamma}|\mathcal{B})\right]\right].\\
\end{split}
\end{equation}
Instead of tackling $\pi(\bm{\beta}, \sigma^2, \delta, \bm{\gamma}|\mathcal{D})$ directly, we propose to iteratively update the lower bound $Q$
\begin{equation}
\begin{split}
\label{obj_expect}
&Q(\bm{\beta}, \sigma, \delta|\bm{\beta}^{(k)}, \sigma^{(k)}, \delta^{(k)})=\E_{\mathcal{B}}\left[\E_{\bm{\gamma}|\mathcal{D}}\left[\log\pi(\bm{\beta}, \sigma^2, \delta, \bm{\gamma}|\mathcal{B})\right]\right].
\end{split}
\end{equation}
Given $(\bm{\beta}^{(k)}, \sigma^{(k)},\delta^{(k)})$ at the k-th iteration, we first sample $\bm{\beta}^{(k+1)}$ from $Q$, then optimize $Q$ with respect to $\sigma, \delta$ and $\E_{\bm{\gamma}_l|\cdot,\mathcal{D}}$ via SA, where $\E_{\bm{\gamma}_l|\cdot,\mathcal{D}}$ is used since $\bm{\gamma}$ is treated as unobserved variable.
% A simplified approach was used for point estimation in a neural-graphical model in a structured prediction task and proved to be useful \citep{Zhang17}.
To make the computation easier, we decompose our $Q$ as follows:
\begin{equation}
\begin{split}
&Q(\bm{\beta},\sigma, \delta|\bm{\beta}^{(k)}, \sigma^{(k)}, \delta^{(k)}) = Q_1(\beta, \sigma|\bm{\beta}^{(k)}, \sigma^{(k)}, \delta^{(k)}) + Q_2(\delta|\bm{\beta}^{(k)}, \sigma^{(k)}, \delta^{(k)})+C,
\end{split}
\end{equation}
Denote $\mathcal{X}$ and  $\mathcal{C}$ as the sets of the indices of sparse and non-sparse layers, respectively. We have:
\begin{equation}
\begin{split}
\label{lab: q1}
&Q_1(\bm{\beta}|\bm{\beta}^{(k)}, \sigma^{(k)},\delta^{(k)})=\underbrace{\frac{N}{n}\log \pi(\mathcal{B}|\bm{\beta})}_\text{log likelihood}-\underbrace{\sum_{l\in \mathcal{C}}\sum_{j\in p_l} \dfrac{\beta_{lj}^2}{2\sigma_0^2}}_\text{non-sparse layers $\mathcal{C}$} -\dfrac{p+\nu+2}{2} \log(\sigma^2)\\
&-\sum_{l\in \mathcal{X}}\sum_{j\in p_l} \underbrace{[\dfrac{|\beta_{lj}|\overbrace{\E_{\bm{\gamma}_l|\cdot,\mathcal{D}} \left[\dfrac{1}{v_0(1-\gamma_{lj})}\right]}^{ \kappa_{lj0}}}{\sigma}+\dfrac{\beta_{lj}^2\overbrace{\E_{\bm{\gamma}_l|\cdot,\mathcal{D}} \left[\dfrac{1}{v_1 \gamma_{lj}}\right]}^{ \kappa_{lj1}}}{2\sigma^2}]}_\text{deep SSGL priors in sparse layers $\mathcal{X}$}- \dfrac{\nu\lambda}{2\sigma^2}
\end{split}
\end{equation}
\begin{equation}
\begin{split}
\label{eq:q2}
&Q_2(\delta_l|\bm{\beta}^{(k)}_l, \delta^{(k)}_l) =\sum_{l\in \mathcal{X}} \sum_{j\in p_l}\log\left(\dfrac{\delta_l}{1-\delta_l}\right) \overbrace{\E_{\gamma_l|\cdot,\mathcal{D}}\gamma_{lj}}^{ \rho_{lj}} + (a-1) \log(\delta_l) + (p_l+b-1) \log(1-\delta_l),
\end{split}
\end{equation}
where $\bm{ \rho}, \bm{ \kappa}$, $\sigma$ and $\delta$ are to be estimated in the next section.
% where $\kappa_{0lj}=\E_{\bm{\gamma}_l|\cdot} \left[\dfrac{1-\gamma_{lj}}{v_0}\right]$, $\kappa_{1lj}=\E_{\bm{\gamma}_l|\cdot} \left[\dfrac{\gamma_{lj}}{v_1}\right]$.

\subsection{Empirical Bayesian via stochastic approximation}

% In linear regression, EMVS \citep{Rockova14} can be used to obtain the point estimates of $\bm{\beta}$ and all the priors. However, when the log likelihood function is non-convex, the radical update of EMVS no longer yields robust hyperparameters. By contrast, a sampling algorithm is more efficient in escaping local traps. 
To simplify the notation, we denote the vector $(\bm{\rho}, \bm{\kappa}, \sigma, \delta)$ by $\bm{\theta}$. Our interest is to obtain the optimal $\bm{\theta}_*$ based on the asymptotically correct distribution $\pi(\bm{\beta}, \bm{\theta}_*)$. This implies that we need to obtain an estimate $\bm{\theta}_*$ that solves a fixed-point formulation $\int g_{\bm{\theta_*}}(\bm{\beta})\pi(\bm{\beta}, \bm{\theta_*})d\bm{\beta}=\bm{\theta}_*$, where $g_{\bm{\theta}}(\bm{\beta})$ is inspired by EMVS to obtain the optimal $\bm{\theta}$ based on the current $\bm{\beta}$. Define the random output $g_{\bm{\theta}}(\bm{\beta})-\bm{\theta}$ as $H(\bm{\beta}, \bm{\theta})$ and the mean field function $h(\bm{\theta}):=\E[H(\bm{\beta}, \bm{\theta})]$. The stochastic approximation algorithm can be used to solve the fixed-point iterations:

\begin{itemize}
\item[(1)] Sample $\bm{\beta}^{(k+1)}$ from a transition kernel $\Pi_{\bm{\theta}^{(k)}}(\bm{\beta})$, which yields the distribution $\pi(\bm{\beta}, \bm{\theta}^{(k)})$,
\item[(2)] Update $\bm{\theta}^{(k+1)}=\bm{\theta}^{(k)}+\omega^{(k+1)} H(\bm{\theta}^{(k)}, \bm{\beta}^{(k+1)})=\bm{\theta}^{(k)}+\omega^{(k+1)} (h(\bm{\theta}^{(k)})+\Omega^{(k)}).$
\end{itemize}
where $\omega^{(k+1)}$ is the step size. The equilibrium point $\bm{\theta}_*$ is obtained when the distribution of $\bm{\beta}$ converges to the invariant distribution $\pi(\bm{\beta}, \bm{\theta}_*)$. The stochastic approximation \citep{Albert90} differs from the Robbins–Monro algorithm in that sampling $\bm{\beta}$ from a transition kernel instead of a distribution introduces a Markov state-dependent noise $\Omega^{(k)}$ \citep{andrieu05}. In addition, since variational technique is only used to approximate the priors, and the exact likelihood doesn't change, the algorithm falls into a class of adaptive SG-MCMC instead of variational inference.


% where $\bm{\theta}$ can be viewed as a vector $(\bm{\rho}, \bm{\tau}, \sigma, \delta)$, the random output $H(\bm{\theta}^{(k)},\bm{\beta}^{(k+1)})$ is equal to 


% To obtain a tight lower bound with respect to the Jensen inequality in (\ref{js_}), we need to obtain an accurate estimation of $\E_{\bm{\gamma}|\cdot, \mathcal{D}}$ (denoted as $\bm{\rho}$). In addition, the lower bound needs to be strictly increasing to converge. However, neither of two conditions are satisfied due to the use of random mini-batch and the non-linear objective functions, which have no close-form update. Instead, we can only estimate $\bm{\gamma}$, $\sigma$ and $\delta$ based on $\mathcal{B}$, this suggests us to approximate $\E_{\gamma|\mathcal{D}}$, $\E[\sigma|\mathcal{D}]$ and $\E[\delta|\mathcal{D}]$ via SA (see details in Appendix A.2).

% The routine for SA to optimize expectation is as follows:




% is defined by is the unbiased estimate of the mean field mapping $h(\hat \theta):=\lim_{k\rightarrow \infty} \E_{\hat \theta}[H(\hat \theta, x_k)]$. When we can sample from $\mu_{{\hat \theta_k}}$ directly and $\mu_{{\hat \theta_k}}$ is in an exponential family, $H(\hat \theta, x)$ is equivalent to the unbiased estimate of the natural gradient of the KL divergence $KL(f_{ \bar \theta}(x)|| f_{\hat \theta_k}(x))$

Regarding the updates of $g_{\bm{\theta}}(\bm{\beta})$ with respect to $\bm{\rho}$, we denote the optimal $\bm{\rho}$ based on the current $\bm{\beta}$ and $\delta$ by $\bm{\tilde\rho}$. We have that $\tilde \rho_{lj}^{(k+1)}$, the probability of $\beta_{lj}$ being dominated by the $L_2$ penalty is
\begin{equation}
\label{eq:10}
\tilde \rho_{lj}^{(k+1)}=\E_{\bm{\gamma}_l|\cdot, \mathcal{B}} \gamma_{lj} = \mathrm{P}(\gamma_{lj}=1|\bm{\beta}_l^{(k)}, \delta_l^{(k)}) =\dfrac{a_{lj}}{a_{lj}+b_{lj}},
\end{equation}
where $a_{lj}=\pi(\beta_{lj}^{(k)}|\gamma_{lj}=1)\mathrm{P}(\gamma_{lj}=1|\delta^{(k)}_l)$ and $b_{lj}=\pi(\beta_{lj}^{(k)}|\gamma_{lj}=0)\mathrm{P}(\gamma_{lj}=0|\delta^{(k)}_l)$. The choice of Bernoulli prior enables us to use $\mathrm{P}(\gamma_{lj}=1|\delta^{(k)}_l)=\delta^{(k)}_l$.


% The physical meaning of $\E_{\bm{\gamma}|\cdot}\gamma_j$ in $Q_2$ is the probability $\rho_j$ that has a large effect on $\beta_j$ in the model, where $\bm{\rho}\in\mathbb{R}^p$.

% When $p$ is large, numerical problems occur in some extremely cases, e.g. $\sigma^2$ decreases sharply. To overcome that issue, we can rewrite
% \begin{equation}
% E_{\gamma|\cdot} \gamma_j =\dfrac{1}{1+b_j/a_j}=\dfrac{1}{1+\dfrac{(1-\delta_{(t)})v_1}{\delta_{(t)} v_0} \exp\{\dfrac{\beta_j^2}{2\sigma^2}(\dfrac{1}{v_1}-\dfrac{1}{v_0})\}}.
% \end{equation}

Similarly, as to $g_{\bm{\theta}}(\bm{\beta})$ w.r.t. $\bm{\kappa}$, the optimal $\tilde \kappa_{lj0}$ and $\tilde \kappa_{lj1}$ based on the current ${\rho_{lj}}$ are given by:
\begin{equation}
\begin{split}
\label{eq:11}
\tilde \kappa_{lj0}&=\E_{\bm{\gamma}_l|\cdot, \mathcal{B}} \left[\dfrac{1}{v_0 (1-\gamma_{lj})}\right]=\dfrac{1- \rho_{lj}}{v_0}; \text{ }\tilde \kappa_{lj1}=\E_{\bm{\gamma}_l|\cdot, \mathcal{B}} \left[\dfrac{1}{v_1 \gamma_{lj}}\right]=\dfrac{ \rho_{lj}}{v_1}.
\end{split}
\end{equation}


% The general strategy of recursion follows ${\beta} \leftarrow \bm{\beta} + \epsilon \nabla_{\bm{\beta}} {\pi}(\bm{\beta}, \sigma^2, \delta|\mathcal{B})$ where $\epsilon$ is the learning rate. 

% , approximation of Eq.(\ref{lab: q1}) is often required, e.g. normal approximation \citep{Gelman13}, VI \citep{Drugowitsch13} or EP \citep{Gelman13}. In deep learning framework, due to the success of

% In order to optimize $Q_1$ with respect to $\sigma$, by denoting $\diag\{\kappa_i\}_{i=1}^p$ as $\bm{\mathcal{V}}$, following the formulation in \citet{McDermott16} and \citet{Rockova14} we have:

% \begin{equation}  
% \label{eq:13}
% \sigma^{(k+1)}=\sqrt{\dfrac{\left\Vert\left(\bm{\mathcal{V}}^{1/2}\bm{\beta}^{(k+1)}\rm\right) \right\Vert^2+ \nu\lambda}{p+\nu+2}}
% \end{equation}

% \begin{equation}  
% \label{eq:13}
% \sigma^{(k+1)}=\left\{  
%              \begin{array}{lr}  
%              \sqrt{\dfrac{\frac{N}{n}\sum_{i\in\mathcal{S}} \left(y_i-\psi(\bm{x}_i;\bm{\beta}^{(k+1)})\right)^2 +||\bm{\mathcal{V}}^{1/2}\bm{\beta}^{(k+1)}||^2+ \nu\lambda}{N+p+\nu}} & \text{(regression)},   \\  
%              \sqrt{\dfrac{\left\Vert\left(\bm{\mathcal{V}}^{1/2}\bm{\beta}^{(k+1)}\rm\right) \right\Vert^2+ \nu\lambda}{p+\nu+2}} &  \text{(classification).}  
%              \end{array}  
% \right.  
% \end{equation}


To optimize $Q_1$ with respect to $\sigma$, by denoting $\diag\{\kappa_{0li}\}_{i=1}^{p_l}$ as $\bm{\mathcal{V}_{0l}}$, $\diag\{\kappa_{1li}\}_{i=1}^{p_l}$ as $\bm{\mathcal{V}_{1l}}$ we have:
\begin{equation}  
\label{eq:13}
\tilde \sigma^{(k+1)}=\left\{  
             \begin{array}{lr}  
             \dfrac{R_b+\sqrt{R_b^2+4R_a R_c}}{2R_a} & \text{(regression)},   \\  
             \dfrac{C_b+\sqrt{C_b^2+4C_a C_c}}{2C_a} &  \text{(classification),}  
             \end{array}  
\right.  
\end{equation}
% \begin{equation}  
% \label{eq:13}
% \sigma^{(k+1)}=\left\{  
%              \begin{array}{lr}  
%              \sqrt{\dfrac{I +J+ \nu\lambda}{N+\sum_{l\in\mathcal{X}}p_l+\nu}} & \text{(regression)},   \\  
%              \sqrt{\dfrac{J+ \nu\lambda}{\sum_{l\in\mathcal{X}}p_l+\nu+2}} &  \text{(classification),}  
%              \end{array}  
% \right.  
% \end{equation}
where $R_a=N+\sum_{l\in\mathcal{X}}p_l+\nu$, $C_a=\sum_{l\in\mathcal{X}}p_l+\nu+2$, $R_b=C_b=\sum_{l\in\mathcal{X}}||\bm{\mathcal{V}}_{0l}\bm{\beta}_l^{(k+1)}||_1$, $R_c=I+J+\nu\lambda$, $C_c=J+\nu\lambda$, $I=\frac{N}{n}\sum_{i\in\mathcal{S}} \left(y_i-\psi(\bm{x}_i;\bm{\beta}^{(k+1)})\right)^2$, $J=\sum_{l\in\mathcal{X}}||\bm{\mathcal{V}}_{1l}^{1/2}\bm{\beta}_l^{(k+1)}||^2$.\footnote[2]{The quadratic equation has only one unique positive root. $\|\cdot\|$ refers to $L_2$ norm, $\|\cdot\|_1$ represents $L_1$ norm.}


To optimize $Q_2$, a closed-form update can be derived from Eq.(\ref{eq:q2}) and Eq.(\ref{eq:10}) given batch data $\mathcal{B}$:
\begin{equation}
\label{eq:14}
\begin{aligned}
\tilde \delta_l^{(k+1)} &= \argmax_{\delta_l \in \mathbb{R}} Q_2(\delta_l|\bm{\beta}_l^{(k)}, \delta_l^{(k)})= \dfrac{\sum_{j=1}^{p_l} \rho_{lj} + a - 1}{a + b + p_l - 2}.
\end{aligned}
\end{equation}


% \subsection{Posterior Approximation and Optimization}
% The posterior average can be approximated through the weighted sample average $\E[\psi(\bm{{\beta}})]=\tfrac{\sum_{k=1}^{{k_{\max}}} \epsilon^{(k)} \psi(\bm{\beta}^{(k)})}{\sum_{k=1}^{{k_{\max}}}\epsilon^{(k)}}$ \citep{Welling11} to reduce the variance of the estimator. \citet{Teh16} showed a theoretical optimal learning rate $\epsilon^{(k)}\propto k^{-1/3}$ for SGLD to achieve faster convergence for posterior average, which is applied in Sec. 6.1.

% To speed up the computation and alleviate the entrapment of latent variables in poor local optima, we can tune $\tau$ to balance between local trap escape and stationary point convergence. This strategy is applied in Sec. 6.2-6.4.


\subsection{Pruning strategy}

There are quite a few methods for pruning neural networks including the oracle pruning and the easy-to-use magnitude-based pruning \citep{Molchanov2016PruningCN}. Although the magnitude-based unit pruning shows more computational savings \citep{Aidan18}, it doesn't demonstrate robustness under coarser pruning \citep{Song16, Aidan18}. Pruning based on the probability $\bm{\rho}$ is also popular in the Bayesian community, but achieving the target sparsity in sophisticated networks requires extra fine-tuning. We instead apply the magnitude-based weight-pruning to our Resnet compression experiments and refer to it as SGLD-SA, which is detailed in Algorithm \ref{alg: SGLD-EM}. The corresponding variant of SGHMC with SA is referred to as SGHMC-SA.

\section{Convergence Analysis}
The key to guaranteeing the convergence of the adaptive SGLD algorithm is to use Poisson's equation to analyze additive functionals. By decomposing the Markov state-dependent noise $\Omega$ into martingale difference sequences and perturbations, where the latter can be controlled by the regularity of the solution of Poisson's equation, we can guarantee the consistency of the latent variable estimators. 
\begin{theorem}[$L_2$ convergence rate]
\label{th:1}
For any $\alpha\in (0, 1]$, under assumptions in Appendix B.1, the algorithm satisfies: there exists a large enough constant $\lambda$ and an equilibrium $\bm{\theta}^*$ such that
\begin{equation*}
\begin{split}
\E\left[\|\bm{\theta}^{(k)}-\bm{\theta}^*\|^2\right]\leq \lambda k^{-\alpha}.
\end{split}
\end{equation*}
\end{theorem}
SGLD with adaptive latent variables forms a sequence of inhomogenous Markov chains and the weak convergence of $\bm{\beta}$ to the target posterior is equivalent to proving the weak convergence of SGLD with biased estimations of gradients. Inspired by \citet{Chen15}, we have:

\begin{corollary}
\label{cor:1}
Under assumptions in Appendix B.2, the random vector $\bm{\beta}^{(k)}$ from the adaptive transition kernel $\Pi_{\bm{\theta}^{(k-1)}}$ converges weakly to the invariant distribution $e^{\tau L(\bm{\beta}, \bm{\theta^*)}}$ as $\epsilon\rightarrow 0$ and $k\rightarrow \infty$.
\end{corollary}

% \begin{corollary}
% \label{cor:1}
% Given fixed stepsize $\epsilon$, the distribution of $\bm{\beta}^{(k)}$ converges weakly to the invariant distribution $e^{\tau L(\bm{\beta}, \bm{\theta}^*)}$ with rate $\alpha\in (0, 1]$ as $\epsilon\rightarrow 0$.
% \end{corollary}

The smooth optimization of the priors
makes the algorithm robust to bad initialization and avoids entrapment in poor local optima. In addition, the convergence to the asymptotically correct distribution enables us to combine simulated annealing \citep{Kirkpatrick83optimizationby}, simulated tempering \citep{ST}, parallel tempering \citep{PhysRevLett86} or (and) dynamical weighting \citep{wong97} to obtain better point estimates in non-convex optimization and more robust posterior averages in multi-modal sampling. %Because SGHMC proposed by \citet{Chen14} is more attractive in large scale problems, the convergence of SGLD-SA also applies to SGHMC-SA.


%If we update $\bm{\beta}$ k iterations, then update the latent variables and then update $\bm{\beta}$ $k$ iterations,..., we call it ESM-k.



% Extension to the $t$-prior is provided in the appendix, where the same framework can be applied.

% \subsubsection{Deterministic annealing to mitigate multimodality}

% To reduce the chances of getting stuck in a local mode, one might use the deterministic annealing variant of the EM algorithm (DAEM) \citep{Ueda98}, which aims to find a minimum of a tempered version of the free energy function, i.e. 

% $H^{(k)}(w, \delta)=\dfrac{1}{t} \log \sum_{\gamma} \pi(\beta, \delta, \gamma, \sigma|y)^t$ \ with $0<t \leq 1$.

% In the above formula, the temperature parameter $1/t$ controls the degree of separation between the multiple modes of $H^{(k)}$. Multiple modes begin to appear as the temperature decreases and $H^{(k)}$ gradually resembles the actual incomplete posterior. Thus the strategy to set a high temperature in the beginning and decrease it later keeps us from the poorly chosen starting values.

% To extend the ESM algorithm to the deterministic annealing ESM iterations, we simply need to adapt the E-step to a modified posterior distribution, which is to replace $p_i^*$ with 
% \begin{equation}
% p_i^t=\dfrac{a_i^t}{a_i^t+b_i^t}=\dfrac{1}{1+[\dfrac{(1-\delta_{(t)})v_1}{\delta_{(t)} v_0} \exp\{\dfrac{\beta^2}{2\sigma^2}(\dfrac{1}{v_1}-\dfrac{1}{v_0})\}]^t},
% \end{equation}
% where $a_j=\pi(\beta_j^{(k)}|\gamma_j=1)P(\gamma_j=1|\delta^{(k)})$ and $b_j=\pi(\beta_j^{(k)}|\gamma_j=0)P(\gamma_j=0|\delta^{(k)})$.




\begin{algorithm}[tb]
   \caption{SGLD-SA with SSGL priors}
   \label{alg: SGLD-EM}
\begin{algorithmic}
   \State {\textbf{Initialize:} $\bm{\beta}^{(1)}$, $\bm{\rho}^{(1)}$, $\bm{\kappa}^{(1)}$, $\sigma^{(1)}$ and $\delta^{(1)}$ from scratch, set target sparse rates $\mathbb{D}$, $\mathbb{f}$ and $\mathbb{S}$}
   \For {$k \leftarrow 1:{k_{\max}}$}
%   \State {Sample mini-batch $\mathcal{B}^{(k)}$}
   \State {\textbf{Sampling}}
%    \State{$\bm{\beta}^{(k+1)}\leftarrow\bm{\beta}^{(k)} + \epsilon^{(k)} \nabla_{\bm{\beta}} {\pi}(\bm{\beta}^{(k)}, \sigma^{(k)}, \delta^{(k)}|\mathcal{B}^{(k)})+\sqrt{2\epsilon^{(k)} T^{-1}}\bm{\eta}^{(k)},\ \where\ \bm{\eta}^{(k)} \sim \mathcal{N}(\bm{0}, \bm{I})$}
   \State {$\bm{\beta}^{(k+1)}\leftarrow\bm{\beta}^{(k)} + \epsilon^{(k)} \nabla_{\bm{\beta}}  Q(\cdot|\mathcal{B}^{(k)})+\mathcal{N}({0, 2\epsilon^{(k)} \tau^{-1}})$}
   
   \State {\textbf{Stochastic Approximation for Latent Variables}}
%   \State {Compute $\bm{\tilde \rho}^{(k+1)}$, $ \bm{\tilde \kappa}^{(k+1)}$, $\tilde \sigma^{(k+1)}$, and $\tilde \delta^{(k+1)}$ according to Eq.(\ref{eq:10}),Eq.(\ref{eq:11}),Eq.(\ref{eq:13}) and Eq.(\ref{eq:14})}.
    % \State {Update the variables following Eq.(\ref{eq:10}),Eq.(\ref{eq:11}),Eq.(\ref{eq:13}) and Eq.(\ref{eq:14})}.
   \State {\textbf{SA}: $\bm{\rho}^{(k+1)}\leftarrow (1-\omega^{(k+1)}) \bm{\rho}^{(k)}+\omega^{(k+1)} \bm{\tilde \rho}^{(k+1)}$ following Eq.(\ref{eq:10})}
   \State {\textbf{SA}: $\bm{\kappa}^{(k+1)}\leftarrow(1-\omega^{(k+1)}) \bm{\kappa}^{(k)}+\omega^{(k+1)} \bm{\tilde \kappa}^{(k+1)}$ following Eq.(\ref{eq:11})}
   \State {\textbf{SA}: ${\sigma}^{(k+1)}\leftarrow (1-\omega^{(k+1)}) {\sigma}^{(k)}+\omega^{(k+1)} {\tilde \sigma}^{(k+1)}$ following Eq.(\ref{eq:13})}
   \State {\textbf{SA}: $\delta^{(k+1)}\leftarrow(1-\omega^{(k+1)}) \delta^{(k)}+\omega^{(k+1)} \tilde \delta^{(k+1)}$ following Eq.(\ref{eq:14})}

   \If {\textbf{Pruning}}
   \State {Prune the bottom-$s\%$ lowest magnitude weights}
    \State {Increase the sparse rate $s\leftarrow \mathbb{S}(1-\mathbb{D}^{k/{\mathbb{f}}})$}
   \EndIf
   \EndFor
\end{algorithmic}
\vspace{0em}
\end{algorithm}

==> NIPS 2019 An Adaptive Empirical Bayesian Method for Sparse Deep Learning -arXiv/sgmcmc.tex <==
%%%%%%%%%%%%%%%%%%% Point Estimates of Deep Neural Network %%%%%%%%%%%%%%%%%%
% \subsection{Bayesian Point Estimates of Deep Neural Network}
% Viewing model $P(y|\bm{x}, W)$ probabilistically, where $W$ are the parameters, inputs $\bm{x}$ of a neural network are mapped onto a high-dimensional space by various layers of affine transformation interleaved with nonlinearities. Maximum likelihood estimation (MLE) with priors is equivalent to maximum a posteriori probability (MAP) estimate in Bayesian statistics:
% \begin{equation}
% \begin{split}
% W^{\MAP} & = \argmax_{W} \log P(W|\mathcal{D}) = \argmax_{W} \log P(\mathcal{D}|W) + \log P(W), \nonumber
% \end{split}
% \end{equation}
% where usually $P(W)$ can be given a Gaussian prior (L2 regularization) or a Laplace prior (L1 regularization).

% \subsection{Stochastic Gradient Langevin Dynamics}

We denote the set of model parameters by $\bm{\beta}$, the learning rate at time $k$ by $\epsilon^{(k)}$, the entire data by $\mathcal{D}=\{\bm{d}_i\}_{i=1}^N$, where $\bm{d}_i=(\bm{x}_i, y_i)$, the log of posterior by $L(\bm{\beta})$. The mini-batch of data $\mathcal{B}$ is of size $n$ with indices $\mathcal{S}=\{s_1, s_2, ..., s_n\}$, where $s_i\in \{1, 2, ..., N\}$. Stochastic gradient $\nabla_{\bm{\beta}} \tilde L(\bm{\beta})$ from a mini-batch of data $\mathcal{B}$ randomly sampled from $\mathcal{D}$ is used to approximate $\nabla_{\bm{\beta}} L(\bm{\beta})$:
\begin{equation}
\begin{split}
\label{factor}
\nabla_{\bm{\beta}} \tilde{L}(\bm{\beta})=\nabla_{\bm{\beta}} \log \mathrm{P}(\bm{\beta})+\dfrac{N}{n}\sum_{i\in \mathcal{S}} \nabla_{\bm{\beta}} \log \mathrm{P}(\bm{d}_i|\bm{\beta}).
\end{split}
\end{equation}
SGLD (no momentum) is formulated as follows:
\begin{equation}
\begin{split}
&\bm{\beta}^{(k+1)}=\bm{\beta}^{(k)} + \epsilon^{(k)} \nabla_{\bm{\beta}} \tilde{L}(\bm{\beta}^{(k)})+\mathcal{N}({0, 2\epsilon^{(k)}\tau^{-1}}),\\
\end{split}
\end{equation}
where $\tau>0$ denotes the inverse temperature. It has been shown that SGLD asymptotically converges to a stationary distribution $\pi(\bm{\beta}|\mathcal{D})\propto e^{\tau L(\bm{\beta})}$ \citep{Teh16,Yuchen17}. As $\tau$ increases and $\epsilon$ decreases gradually, the solution tends towards the global optima with a higher probability. Another variant of SG-MCMC, SGHMC \citep{Chen14, yian2015}, proposes to generate samples as follows:
\begin{equation}  
\label{undampedsgld}
\left\{  
             \begin{array}{lr}  
             d \bm{\beta}=\bm{r}dt,  \\  
              & \\
%              \prod_{i=1}^{m} \psi(\bm{x_i};\bm{\beta})^{y_i} \left(1-\psi(x_i;\bm{\beta})\right)^{1-y_i}, &  \text{classification}  
             d\bm{r}=\nabla_{\bm{\beta}} \tilde{L}(\bm{\beta})dt-\bm{C}\bm{r}dt+\mathcal{N}(0, 2\bm{B}\tau^{-1}dt)+\mathcal{N}(0, 2(\bm{C}-\bm{\hat{B}})\tau^{-1}dt),   
             \end{array}  
\right.  
\end{equation} 
where $\bm{r}$ is the momentum item, $\bm{\hat{B}}$ is an estimate of the stochastic gradient variance, $\bm{C}$ is a user-specified friction term. Regarding the discretization of (\ref{undampedsgld}), we follow the numerical method proposed by \citet{Saatci17} due to its convenience to import parameter settings from SGD.


% \subsection{Being Bayesian by Backpropagation}
% Bayesian inference for neural networks calculates the posterior distribution of the weights, \citet{Hinton93,Graves11} suggested to minimize the Kullback-Leibler (KL) divergence between the approximating distribution and the true Bayesian posterior on the weights:
% \begin{equation}
% \begin{split}
% \delta^*&= \argmin_{\delta} \mathcal{KL}[q(\w|\delta) || p(\w|\mathcal{D})] \\
%   & \propto \argmin_{\delta} \mathcal{KL}[q(\w|\delta)||p(\w)] -E_{q(\w|\delta)}[\log p(\mathcal{D}|\w)].
% \end{split}
% \end{equation}
% Since the minimization of the cost function in (1) is computational extensive, gradient descent and approximations are used in general.

% To deal with $E_{q(\w|\delta)}[\log p(\mathcal{D}|\w)]$ in (1), \citet{Blundell15} proposed a variational inference (VI) method, called $Bayes\ by\ Backprop$. The number of parameters is doubled by assuming $\w \sim \mathcal{N}(\mu, \sigma)$, which leads to the variational posterior $\delta=(\mu, \rho)$ where $\sigma=\log(1+\exp(\rho))$. The posterior optimization proceeds as follows
% \begin{equation}
% \begin{split}
% \Delta_{\mu}&=\dfrac{\partial f(\w, \delta)}{\partial \w} + \dfrac{\partial f(\w, \delta)}{\partial \mu} \\
% \Delta_{\rho}&=\dfrac{\partial f(\w, \delta)}{\partial \w}\dfrac{\epsilon}{1+\exp(-\rho)} + \dfrac{\partial f(\w, \delta)}{\partial \rho}. \nonumber
% \end{split}
% \end{equation}

% A scale Gaussian mixture prior with zero mean and different variances is also proposed to make the prior more amenable during optimization, experiments on its comparison with dropout showed the slow convergence. In addition, the uncertainty test in the weights from $q(\w|\delta)$ are discussed in regression problems.


% %%%%%%%%%%%%%%%%%%%%% Black-box alpha-divergence %%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Black-box \texorpdfstring{$\alpha$}-divergence}

% Dropout is widely used in DNN as a stochastic regularization technique \citep{Hinton12,Srivastava14}. The theoretical explanation of dropout \citep{Gal16b} relates it to an approximation of the probabilistic deep Gaussian process \citep{Damianou13}. The prediction uncertainty is introduced by the uncertainty of the weights by marginalizing over the approximate posterior using Monte Carlo integration \citep{Gal16a,Gal16b}.

% However, dropout variation inference \citep{Gal16a,Gal16b,Gal17} underestimates model uncertainty which is harmful to AI safety applications. A good alternative is to use black-box $\alpha$-divergence minimization \citep{Hernandez-Lobato16,Li16}.

% Consider the following approximating distribution:
% \begin{equation}
% p(\w)=\dfrac{1}{Z} p_0(\w) \prod_{n} f_n(\w). \nonumber
% \end{equation}
% Variational inference (VI) \citep{Jordan99} and expectation propagation (EP) \citep{Minka01} have been shown to be special cases of power EP \citep{Minka04} that minimizes Amari's $\alpha$-divergence \citep{Amari85}. 
% \begin{equation}
% D_{\alpha}[p||q]=\dfrac{1}{\alpha (1-\alpha)} (1-\int p(\w)^{\alpha} (1-p(\w))^{1-\alpha}d\w), \nonumber
% \end{equation}
% where $\alpha=0$ is used in VI, $\alpha=0.5$ corresponds to the Hellinger distance, $\alpha=1$ is used in EP.

% To make BB-$\alpha$ energy applicable for dropout and other flexible approximation structures, the BB-$\alpha$ energy is simplified as \citep{Li17}.
% \begin{equation}
% \mathcal{L}(q) \approx \mathcal{KL}[q||p_0]-\dfrac{1}{\alpha} \sum_{n} \log E_q[f_n(\w)^{\alpha}]. \nonumber
% \end{equation}
% Approximation to $E_q[\cdot]$ can be handle through Monte Carlo sampling by simply passing the input through the dropout network multiple times through the new BB-alpha loss function.
% Experiments showed that $\alpha=1$ is more robust to adversarial attacks, but less effective in point estimation compared to the other metrics $\alpha=0$ and $\alpha=0.5$.

==> convergence.tex <==


% % Uncertainty quantification of large systems is extremely time-consuming. In the framework of deep neural networks, it is necessary to propose an efficient sampling method for Bayesian deep learning models with latent variables. It is natural to use a Gibbs sampler in SGLD to sample latent variables $\bm{H}$ in sequence (\ref{eq:17}) and obtain an "auxiliary" ergodic Markov Chain \citep{George93}: 
% % \begin{equation}
% % \label{eq:17}
% % \bm{\beta}^{(1)}, \bm{H}^{(1)}; \bm{\beta}^{(2)}, \bm{H}^{(2)}; \bm{\beta}^{(3)}, \bm{H}^{(3)}; \ldots
% % \end{equation}
% % However, this strategy has been criticized \citep{Rockova14} due to its lack of efficiency in sampling and practicality in large-scale problems. 

% In this section, we study the convergence of the algorithm when the network is not pruned, we view $(\bm{\rho}, \sigma, \bm{\tau}, \delta)$ as a vector $\bm{\theta}$ and formulate our algorithm as follows: % Liang's version
% % Extension of EMVS to DNN is nontrivial since we cannot get the closed form solution of $\bm{\beta}$ as in EMVS. In addition, the improper initialization of hyperparameters and the noise from stochastic optimization error strongly bias the updates of latent variables, which either causes them to rapidly converge to arbitrarily poor local optima or makes the whole algorithm diverge. To tackle this issue, we replace the M-step by SG-MCMC with the prior hyperparameters tuned via stochastic approximation \citep{Albert90} (Appendix A.2): % Liang's version % Liang, Deng's combination
% % Extension of EMVS to DNN is nontrivial since we cannot get the closed form solution of $\bm{\beta}$ as in EMVS. In addition, the improper initialization of hyperparameters and the noise from stochastic optimization error strongly bias the updates of latent variables, which either causes them to rapidly converge to arbitrarily poor local optima or makes the whole algorithm diverge. To make sure the convergence of SG-MCMC in models with latent variables, we propose to use the idea of stochastic approximation \citep{Albert90} (see details in Appendix A.2) to control the growth of approximation error by iteratively updating the latent variables: % Deng's version
% \begin{equation}
% \begin{split}
% \label{eq:0000}
% \bm{\beta}^{(k+1)}&=\bm{\beta}^{(k)} + \epsilon^{(k)} \nabla_{\bm{\beta}} \tilde{L}(\bm{\beta}^{(k)}, \bm{\theta}^{(k)})+\tilde{\bm{\eta}}^{(k)}, \\
% \bm{\theta}^{(k+1)}&=\bm{\theta}^{(k)}+\omega^{(k+1)}\left( g_{\bm{\theta}^{(k)}}(\bm{\beta}^{(k+1)})-\bm{\theta}^{(k)}\right), \\
% \end{split}
% \end{equation}
% where $\tilde{\bm{\eta}}^{(k)}\sim\mathcal{N}(0, 2\epsilon^{(k)}/\tau\bm{I})$,  $g_{\bm{\theta}}(\cdot)$ is the mapping detailed in Eq.(\ref{eq:10}), Eq.(\ref{eq:11}), Eq.(\ref{eq:13}) and Eq.(\ref{eq:14}) to derive $\bm{\theta}$ based on the current $\bm{\beta}$, the step size $\omega^{(k)}$ can be set as $A(k+Z)^{-\alpha}$ with $\alpha\in (0.5, 1]$. The interpretation of this algorithm is that we sample $\bm{\beta}^{(k+1)}$ from $\tilde{L}(\bm{\beta}^{(k)}, \bm{\theta}^{(k)})$ and adaptively optimize the expectation of $\bm{\theta}^{(k+1)}$. 
% % We expect to obtain an augmented sequence as follows: 
% % \begin{equation}
% % \label{eq:17}
% % \bm{\beta}^{(1)}, \bm{\theta}^{(1)}; \bm{\beta}^{(2)}, \bm{\theta}^{(2)}; \bm{\beta}^{(3)}, \bm{\theta}^{(3)}; \ldots
% % \end{equation}

% To provide the $L^2$ upper bound for SGLD-SA, we first lay out the following assumptions:
% \begin{assumption}[Step size]
% \label{ass1}
% $\{\omega^{(k)}\}_{k\in \mathrm{N}}$ is a positive decreasing sequence of real numbers such that
% \begin{equation}
% \begin{split}
% \label{a1}
% &\omega^{(k)}\rightarrow 0, \ \ \sum_{k=1}^{\infty} \omega^{(k)}=+\infty.
% \end{split}
% \end{equation}
% \end{assumption}

% \begin{assumption}[Smoothness]
% \label{ass_2_1}
% $L(\bm{\beta}, \bm{\theta})$ is $G$-smooth with $G>0$, i.e. for any $\bm{\beta}, \bm{\iota}\in \bm{B}$, $\bm{\theta}, \bm{\upsilon}\in\bm{\Theta}$.
% \begin{equation}
% \begin{split}
% \label{ass_2_1_eq}
% \|\nabla_{\bm{\beta}} L(\bm{\beta}, \bm{\theta})-\nabla_{\bm{\beta}} L(\bm{\iota}, \bm{\upsilon})\|\leq G\|\bm{\beta}-\bm{\iota}\|+G\|\bm{\theta}-\bm{\upsilon}\|. 
% \end{split}
% \end{equation}
% \end{assumption}

% \begin{assumption}[Dissipative] There exist constants $m>0, b\geq 0$, s.t. for all $\bm{\beta} \in \bm{\beta}$ and $\bm{\theta} \in \bm{\Theta}$, we have 
% \label{ass_dissipative}
% \begin{equation}
% \label{eq:01}
% \langle \nabla_{\bm{\beta}} L(\bm{\beta}, \bm{\theta}), \bm{\beta}\rangle\leq b-m\|\bm{\beta}\|^2.
% \end{equation}
% \label{as:2_2}
% This condition is essential to induce ergodicity.  \citep{mattingly02, Xu18}, which means that a Markov process is able to move inwards on average.
% \end{assumption}

% \begin{assumption}[Gradient condition] The stochastic noise $\bm{\chi}^{(k)}$, which equals $\nabla_{\bm{\beta}}\tilde L(\bm{\beta}^{(k)}, \bm{\theta}^{(k)})-\nabla_{\bm{\beta}} L(\bm{\beta}^{(k)}, \bm{\theta}^{(k)})$, is a white noise and is independent with each other.
% \begin{equation}
% \begin{split}
% \label{eq:19}
% \E[\bm{\chi}^{(k)}|\mathcal{\bm{F}}^{(k)}]&=0.\\
% \end{split}
% \end{equation}
% For constants $M, B>0$, the noise scale is bounded by
% \begin{equation}
% \begin{split}
% \label{eq:19_11}
% \E\|\bm{\chi}\|^2 \leq M\E\|\bm{\beta}\|^2+M\E\|\bm{\theta}\|^2+B.\\
% \end{split}
% \end{equation}
% \label{as:1}
% \vspace{-2em}
% \end{assumption}
% We then show that both $\bm{\beta}$ and $\bm{\theta}$ are bounded in $L^2$ and present the details in Appendix B.1. 
% \begin{lemma}[Uniform $L^2$ bound]
% \label{lemma:1}
% For all $\ 0<\epsilon<\operatorname{Re}(\tfrac{m-\sqrt{m^2-2M(M+1)}}{2M(M+1)})$, there exist $G, \overline{G}>0$ such that
% $\sup \E\|\bm{\beta}_k\|^2 \leq G$ and $\sup \E\|\bm{\theta}_k\|^2 \leq \overline{G}$, where $G=\|\bm{\beta}_0\|^2 + \tfrac{1}{m}(b+B(M+1)+\tau d)$ and $\overline{G}=MG+B$.\footnote{Here we assume $\bm{\beta}\in \mathbb{R}^d$}
% \end{lemma}

% The uniform $L^2$ bound is crucial to show the convergence for the latent variables.

% \begin{theorem}[$L^2$ convergence rate]
% \label{th:1}
% For any $\alpha\in (0, 1]$, under assumptions in Appendix B.1, the algorithm satisfies: there exists a constant $\lambda$ such that
% \begin{equation*}
% \begin{split}
% \E\left[\|\bm{\theta}^{(k)}-\bm{\theta}^*\|^2\right]\leq \lambda\omega^{(k)},
% \end{split}
% \end{equation*}
% \end{theorem}
% where $\omega^{(k)}=A(k+Z)^{-\alpha}$ for some positive $A$ and $Z$.

% \begin{corollary}
% \label{cor:1}
% Given fixed stepsize $\epsilon$, the distribution of $\bm{\beta}^{(k)}$ converges weakly to the invariant distribution $e^{\tau L(\bm{\beta}, \bm{\theta}^*)}$ with rate $\alpha\in (0, 1]$ as $\epsilon\rightarrow 0$.
% \end{corollary}

% The key to guaranteeing the consistency of the latent variable estimators is from the theory of SA and the fact of $\sum_{i=1}^{\infty} \omega^{(i)}=\infty$. The smooth update of the latent variables makes the algorithm robust to bad hyperparameters and is more likely to avoid entrapment in poor local optima. The non-convex optimization of SG-MCMC \citep{Maxim17, Yuchen17, Xu18} with suitable temperature or cooling schedules ensures the robust optimization of the latent variables. Because SGHMC proposed by \citet{Chen14} is essentially a second-order Langevin dynamics and yields a stationary distribution given an accurate estimation of the error variance from the stochastic gradient, the convergence of SGLD-SA also applies to SGHMC-SA.


% \begin{algorithm}[tb]
%    \caption{SGLD-SA with spike and slab priors}
%    \label{alg: SGLD-EM}
% \begin{algorithmic}
%    \State{\textbf{Inputs:} $\{\epsilon^{(k)}\}_{k=1}^{\mathcal{T}}$, $\{\omega^{(k)}\}_{k=1}^{\mathcal{T}}$, $\tau$, a, b, $\nu$, $\lambda$, $v_0$, $v_1$}
%    \State{\textbf{Outputs:} $\{\bm{\beta}^{(k)}\}_{k=1}^{\mathcal{T}}$}
%    \State{\textbf{Initialize:} $\bm{\beta}^{(1)}$, $\bm{\rho}^{(1)}$, $\bm{\kappa}^{(1)}$, $\sigma^{(1)}$ and $\delta^{(1)}$ from scratch}
%    \For{$k \leftarrow 1:\mathcal{T}$}
%    \State{Sample mini-batch $\mathcal{B}^{(k)}$}
%    \State{\textbf{Sampling}}
% %    \State{$\bm{\beta}^{(k+1)}\leftarrow\bm{\beta}^{(k)} + \epsilon^{(k)} \nabla_{\bm{\beta}} {\pi}(\bm{\beta}^{(k)}, \sigma^{(k)}, \delta^{(k)}|\mathcal{B}^{(k)})+\sqrt{2\epsilon^{(k)} T^{-1}}\bm{\eta}^{(k)},\ \where\ \bm{\eta}^{(k)} \sim \mathcal{N}(\bm{0}, \bm{I})$}
%    \State{$\bm{\beta}^{(k+1)}\leftarrow\bm{\beta}^{(k)} + \epsilon^{(k)} \nabla_{\bm{\beta}}  Q(\bm{\beta}, \sigma, \delta|\bm{\beta}^{(k)}, \sigma^{(k)}, \delta^{(k)})+\mathcal{N}({0, 2\epsilon^{(k)} \tau^{-1}})$}
%    \State{\textbf{Optimization}}
%    \State{Compute $\bm{\rho}^{(k+1)}$ in Eq.(\ref{eq:10}), perform SA: $\bm{\rho}^{(k+1)}\leftarrow (1-\omega^{(k+1)}) \bm{\rho}^{(k)}+\omega^{(k+1)} \bm{\rho}^{(k+1)}$}
%    \State{Compute $\bm{\kappa}^{(k+1)}$ in Eq.(\ref{eq:11}), perform SA: $\bm{\kappa}^{(k+1)}\leftarrow (1-\omega^{(k+1)}) \bm{\kappa}^{(k)}+\omega^{(k+1)} \bm{\kappa}^{(k+1)}$}
%    \State{Compute $\sigma^{(k+1)}$ in Eq.(\ref{eq:13}), perform SA: $\sigma^{(k+1)}\leftarrow(1-\omega^{(k+1)}) \sigma^{(k)}+\omega^{(k+1)} \sigma^{(k+1)}$}
%    \State{Compute $\delta^{(k+1)}$ in Eq.(\ref{eq:14}), perform SA: $\delta^{(k+1)}\leftarrow(1-\omega^{(k+1)}) \delta^{(k)}+\omega^{(k+1)} \delta^{(k+1)}$}
%    \EndFor
% \end{algorithmic}
% \end{algorithm}


==> relworks.tex <==
% \begin{corollary}
% Given fixed stepsize $\epsilon$, the distribution of $\bm{\beta}^{(k)}$ from SG-MCMC-SA converges weakly to the invariant distribution $\pi(\bm{\beta}, \bm{\rho}^{*}, \bm{\kappa}^{*}, \delta^*|\mathcal{D})$ with rate $\alpha\in (0, 1]$ as $\epsilon\rightarrow 0$.
% \end{corollary}


% \citet{Teh14,Chen15} also pointed out that SGHMC has an optimal stepsize $\epsilon \propto K^{-1/3}$ with respect to the bias of the expected sample average and $\epsilon \propto K^{-1/5}$ with respect to MSE in the $K$-th iteration. When considering the practical issue of limited time, since the polynomial-decay learning rate decreases very fast in the early phase, it can potentially influence the efficiency. To overcome that issue, \citet{Welling11} kept a constant stepsize once the stepsize decreased below a critical level; \citet{Chen14} used a small fixed $\epsilon$ to gain efficiency. We instead seek a balance between fixed value and polynomial decay and use an exponential decay $(1-0.001)^K$ to mildly decrease the stepsize in the early phase.

% In addition, in Hamiltonian dynamics, given injected noise variance $M$, the kinetic energy is usually defined as $K(p)=p^TM^{-1}p/2$ \citep{Neal10}, whereas in the backprop based DNN, we found that $K(p)=p^Tp/2$ achieves a much faster mixing without violating the reversibility and conservation. The proof is similar to \citet{Neal10} and is omitted in this paper. This leads to a modification of SGHMC from letting $v\sim \mathcal{N}(0, \epsilon I)$, $\Delta v=-\epsilon^2M^{-1}\Delta U(\delta)-\epsilon M^{-1}Cv +\mathcal{N}(0, 2\epsilon^3M^{-1}(C-\hat B)M^{-1})$ to the following equation
% \begin{equation}
% \begin{split}
% &letting\ v\sim \mathcal{N}(0, \epsilon V_l) \\
% &\Delta\delta = v \\
% &\Delta v=-\epsilon^2\Delta U(\delta)-\epsilon Cv +\mathcal{N}(0, 2\epsilon^3(C-\hat B)).
% \end{split}
% \end{equation}

% In our model, $V_l$ is estimated from empirical Fisher information $V_l=\dfrac{\sum_{k=1}^{p_l} (\pi_{\beta_{(t)}}-\bar\pi_{\beta_{(t)}})^2}{p_l-1}$  for each layer $l$\ \citep{Ahn12}. In the sparse weights, to account for the different variances for different weights, we can modify $V_l$ to be $V_l=E(\Sigma_l)$, where $E_{\beta_j}(\Sigma_l)=(\sigma^*)^2 [v_0 (1-p_j^*) + v_1 p_j^*]$. If we further assume $\alpha=\epsilon C$, $\eta=\epsilon^2$, $b=\epsilon \hat B$, the implementation details are shown in Algorithm 1. We refer to the SGHMC pretrained with ESM framework as \textbf{sSGHMC}.
Dropout alleviates over-fitting and provides an efficient way of making bagging practical for ensembles of countless sub-networks. It can be interpreted as assigning mixture priors on the hidden units \citep{Yarin16b}.
From the Bayesian perspective, our proposed algorithm differs from Dropout and its variants in treating the priors: our algorithm keeps updating the priors during posterior inference, rather than keep them fixed. The inclusion of scaled mixture priors in deep learning models were also studied in \citet{Blundell15,Li16} with encouraging results. 

Our algorithm shares some similarities with variational Bayes (VB) and EMVS, such as the efficiency and the lower bound approximation, but differs from them 
fundamentally. First, our proposed algorithm only approximates the latent variables, while sampling the weights via SG-MCMC. Second, EMVS, mainly designed for linear models with closed-form update, doesn't work for highly non-linear DNN models lacking closed-form solution. In addition, it is unable to optimize the latent variables stochastically. A trivial implementation of EMVS in DNNs will likely cause the latent variables to trap in poor local optima.

Our setup differs from Bayesian Elastic Net \citep{li2010, hans11} and mixed shrinkage prior \citep{Georgios14} in that our model not only is self-adaptive but also yields a more efficient framework for inference.

%The use of numerical differentiation implicitly allows the pruned values to be able to change their value if they become important again. %Due to the rapid development of automatic differentiation, we are not concerned with the problem when the weights $\bm{\beta}$ are mathematically not differentiable at 0.


% Inspired by MCMC model composition ($MC^3$) by \citet{Madigan94}, the presence of model uncertainty enables us to achieve better performance in point estimation through BMA \citep{Welling11,Li16} from MCMC samples. If we simulate Markov Chain $\beta(t), t=1,2,\ldots, N$ from invariant distribution $\pi(\beta^{(k)}|\mathcal{D})$, then the weigted average (Welling, M., 2011) $\dfrac{\sum_{t=1}^{N} \epsilon^{(k)} \psi(\beta^{(k)})}{\sum_{t=1}^{N}\epsilon^{(k)}}$ converges to  $E[\psi(\hat \beta)]$ as $N \rightarrow \infty$. we refer to \textbf{sSGHMC} with BMA as \textbf{esSGHMC}. 

% \begin{algorithm}[tb]
%    \caption{Posterior Sampling with spike-and-slab prior: $\epsilon$ is the stepsize, $\eta=\epsilon^2$ is the learning rate, $\alpha$ corresponds to the friction term, $p_l$ is the number of parameters in layer $l$, $\pi_{\beta}$ is the posterior derivative with respect to $\beta$. In practice, $\alpha=0.01$, $b=\dfrac{1}{2}\eta$, $\kappa=0.001$, L=5}
% \begin{algorithmic}
%    \Require{mini-batch $\mathcal{D}$}
%    \State{Initialize $\beta$, $\sigma$ and $p$ from scratch or ESM}
%    \For{$K$ in $1, 2, ..., m$}
%    \State{$\epsilon \leftarrow \epsilon-\kappa \epsilon$; $\eta\leftarrow\epsilon^2$}
%    \For{each layer $l$}
%    \If{weights are sparse}
%    \State{$V_l=E_{\beta}(\Sigma_l)$}
%    \Else
%    \State{$V_l=\dfrac{\sum_{k=1}^{p_l} (\pi_{\beta_{(t)}}-\bar\pi_{\beta_{(t)}})^2}{p_l-1}$}
%    \EndIf
%    \State{Sample $v \sim \epsilon \mathcal{N}(0, V_l)$}
%    \For{each leapfrog $1, 2, \ldots, L$}
%    \State{$\beta \leftarrow \beta + v$}
%    \State{$v \leftarrow (1-\alpha) v - \eta \pi_{\beta}(\beta, \sigma^*, \gamma|\mathcal{D}) + 2(\alpha-b)\eta\mathcal{N}(0, V_l)$}
%    \EndFor
%    \EndFor
%    \State{Append $\beta$ to the chains}
%    \EndFor
% \end{algorithmic}
% \end{algorithm}

% \subsection{Comparison with DropConnect}

% Binary DropConnect \citep{Liwan13} and our proposed algorithm both assume the spike-and-slab prior on the weights. The difference is that the former doesn't update the prior parameters during inference while the later one does.
